ICMarks: A Robust Watermarking Framework for Integrated Circuit Physical Design IP Protection

Physical design watermarking on contemporary integrated circuit (IC) layout encodes signatures without considering the dense connections and design constraints, which could lead to performance degradation on the watermarked products. This paper presents ICMarks, a quality-preserving and robust watermarking framework for modern IC physical design. ICMarks embeds unique watermark signatures during the physical design's placement stage, thereby authenticating the IC layout ownership. ICMarks's novelty lies in (i) strategically identifying a region of cells to watermark with minimal impact on the layout performance and (ii) a two-level watermarking framework for augmented robustness toward potential removal and forging attacks. Extensive evaluations on benchmarks of different design objectives and sizes validate that ICMarks incurs no wirelength and timing metrics degradation, while successfully proving ownership. Furthermore, we demonstrate ICMarks is robust against two major watermarking attack categories, namely, watermark removal and forging attacks; even if the adversaries have prior knowledge of the watermarking schemes, the signatures cannot be removed without significantly undermining the layout quality.

==> files_backup/1_intro.tex <==
In the modern very-large-scale integrated circuit (VLSI) supply chain, companies across multiple countries collaborate to design, fabricate, assemble, and verify integrated circuits (ICs)~\cite{liu2016vlsi,pawar2018risks,harrison2021malicious}.
The final product integrates intellectual property (IP) components from various stakeholders, including design and fabrication houses, threaded along the global supply chain. With the confluence of such diverse inputs, safeguarding IP emerges as an undeniable urgent, particularly to preempt IP piracy threats\cite{shamsi2019ip,knechtel2019protect,slpsk2023treehouse}. 
As part of the supply chain, the physical design bridges the logic design with the VSLI layouts for manufacturing. The final layouts strategically optimize the positioning and connectivity of components on the chip canvas, leading to reductions in power consumption and area utilization. This not only translates into million-dollar manufacturing cost savings for chip producers but also establishes invaluable IPs. However, they are vulnerable to potential exploitation like overbuilding and counterfeiting from untrusted third parties in the supply chain, emphasizing the urgency for robust protective measures.


%The well-designed layouts optimize the chip to reduce power consumption, area utilization, etc., saving chip producers millions of dollars in manufacturing costs and constituting pivotal IPs. 




%%\racheltodo{Introduce the stages briefly before narrowing to placement stage in physical design. It would be good to include figure 1 for this.}
%The final product integrates IPs from various providers on the long IC supply chain, where the IP of each provider needs to be protected.  
%An important IP in the chip design flow is placement~\cite{lin2019dreamplace,mirhoseini2021graph,gu2020dreamplace}, which is the initial step for physical design, and significantly influences the power consumption, performance, and efficiency of design products.
%Several protection methods such as design obfuscation~\cite{narayanan2006limits,brakerski2014black,zhang2017dynamically,zhang2018chip,shamsi2019ip} and VLSI fingerprinting~\cite{caldwell1999effective,qu2000fingerprinting,prabhu2011extracting,stern2019emforced} have been introduced. These techniques are primarily tailored for routing or partition-based placement, thereby failing to provide proof of ownership for VLSI placements generated by modern analytical-based algorithms. 
%A promising set of solutions for safeguarding physical design IP is provided by embedding watermark signatures.
%Generally speaking, inserting watermarks in the VLSI layout presents several challenges.
%\ruisi{ }%The row parity watermarking~\cite{kahng2001constraint} does not account for the additional constraints during watermarking, resulting in diminished performance on certain benchmarks.

Watermarking~\cite{rathor2023hard,chen2023intellectual,tauhid2023survey} has emerged as a viable methodology to safeguard physical design IP by embedding unique signatures into the IC layouts. These watermarks, derived from unique and confidential identifiers, are embedded into the layouts. They are inconspicuous upon inspection and do not impact the IC's overall quality. To authenticate ownership, the design houses verify the watermark signatures by extracting the watermarks from the IC layout. 

%Existing physical design watermarking frameworks proposed to insert watermarks in the placement or routing stages.
%The placement watermarking-based approach named Row Parity~\cite{kahng2001constraint} inserts signatures by modifying the row index, where the row identifier of watermarked cells represents unique signatures via bit sequences. Though the placement watermarking scheme guarantees $100\%$ watermark extraction rate, these techniques do not consider new constraints, such as fence regions and macros, that could lead to IC performance degradation. On the other hand, routing-based watermarks add redundant bends to insert as signatures, substantially increasing the overall wirelength cost~\cite{1510323}. %Besides, all these physical design watermarking schemes are susceptible to the ghost watermark attack, where adversaries with access to the design layout can implement another set of similar watermarks and claim ownership of the IC.


Nevertheless, inserting watermarks into modern IC layouts is non-trivial and exhibits several challenges. First, large-scale designs have dense standard cell connections, and slight perturbations of the cell locations can degrade the overall performance. Second, modern ICs often have additional design constraints like fence regions and macros. Designing watermarking algorithms without considering these additional design constraints will affect overall performance on certain benchmarks. Finally, the watermarks should be robust against various potential real-world attacks from the supply chain. 

Existing physical design watermarking frameworks proposed to insert watermarks during the placement or routing stages in the physical design process. The placement-based watermarking approach named Row Parity~\cite{kahng2001constraint} inserts signatures by modifying the row index. The watermarked cells' row identifiers represent signatures via binary sequences.  Though the placement watermarking scheme guarantees $100\%$ watermark extraction rates, these techniques do not consider new constraints in modern VLSI design, such as fence regions and macros, that could lead to IC performance degradation. On the other hand, routing-based watermarks add redundant bends to insert as signatures, which substantially increases the overall wirelength cost~\cite{1510323}. Furthermore, no systematic robustness assessments have been performed on those watermarking frameworks, casting doubts over their resilience against real-world adversaries.
%} \ruisi{identifies regions and associated cells that undergo minimal performance deterioration after watermark embedding via a customizedscoring function.}


%The watermark region and cells within the region are added as a co-optimization term in global placement and legalization to enforce watermark insertion. %is introduced prior to the detailed placement to %

This paper devises \sys{}, a novel effective approach to safeguard IC layout IP through placement watermarking. \sys{} demonstrates no performance degradation after watermark insertion and exhibits robustness against a spectrum of attacks. Generally, the placement phase encompasses three integral submodules: global placement, legalization, and detailed placement. \sys's watermarks are integrated into both global and detailed placement modules. It consists of two consecutive steps: 
(i) \textit{Global Watermarking} (GW) leverages a customized scoring scheme to identify the watermarked region and its associated cells, establishing GW signatures without compromising placement quality;
(ii) Next, \textit{Detailed Watermarking} (DW)
inserts unique and confidential signatures on top of the watermarked region from GW. They are infused into the watermarked region by moving selected watermarked cells in the region along both the x- and y-directions.
%The placement quality and the following VSLI layout quality are preserved by inserting watermarks on the regions that cause minimal performance degradation identified by the customized scoring scheme from GW.
To verify the existence of signatures in the IC layout, \sys{} first extracts cells in the watermarked region and computes a watermark extraction rate for GW.
Then, the selected watermarked cell positions within the watermarked region are compared with the DW signatures to obtain a watermark extraction rate for DW. The two GW and DW watermarks collaboratively intensify the watermark strength. 


To evaluate the resilience of \sys{} against threats within the real-world supply chain, we classify the potential attacks into three categories:  \textit{Ghost Attacks}, where the adversary extracts an alternative \textit{ghost watermark} from the layout, and claim his ownership with the \textit{ghost watermark}; \textit{Denial Attacks}, wherein the adversary claims the watermarks' presence in the layout is coincidental;  and \textit{Removal Attacks}, where adversary alters cells in the layout to removes the embedded watermarks from the design company. Extensive evaluations have demonstrated the robustness of \sys{} under all aforementioned attacks. In brief, our contributions are as follows:


%To scan the robustness of \sys from real-world supply chain threats, we systematically classify potential attacks into three categories based on attack scenarios: \textit{Ghost Attacks}, where adversaries counterfeit alternative watermarks from the design as \textit{ghost watermarks}; \textit{Denial Attacks}, where adversaries overbuild the layout by claiming the watermarks are coincidental and sell the original copy to users; and \textit{Removal Attacks}, where adversaries overbuild the layout by removing the embedded watermarks. Extensive evaluations have demonstrated the robustness of \sys{} under all aforementioned attacks. 


%The region extraction rate helps determine if a specific owner produces the placement. By calculating the cell extraction rate, the owner can include unique and confidential signatures, thereby augmenting the strength of the watermark.
%The subsequent detailed placement compensates for the performance degradation that originated from the watermark insertion, ultimately resulting in the watermarked placement with a minimal quality degradation.
%\racheltodo{I've commented out the details on which placement stage the watermarks are introduced. I did this because you haven't introduced placement or the different stages yet and to a reader without knowledge about placement it would not make sense.}

\begin{itemize}
    \item We present \sys, a robust watermarking scheme for the modern VLSI physical design pipeline, which does not degrade the layout quality while preserving $100\%$ watermark extraction rates.
    \item \sys{} employs a two-level watermarking approach to ensure minimal performance degradation. \textit{Global Watermarking} identifies the watermarked region and associated cells with minimal quality deterioration to insert signatures, while \textit{Detailed Watermarking} perturbs the cells on top of the GW watermarked region to strengthen the watermarks. 
  %  \racheltodo{Here we only say that GW identifies region to watermark and DW inserts the signature. How does GW-only scheme watermark the cells in the selected region?}
  %   \item Extensive experiments on the ISPD'2005, ISPD'2015, and ISPD'2019 benchmark suites demonstrate that \sys{} successfully inserts watermarks without degrading estimated placement wirelength and routed wirelength. While the best-practicing baseline approach~\cite{kahng2001constraint} incurs an average of 0.44\% estimated placement wirelength and 1.56\% routed wirelength deterioration. 
    \item  Extensive experiments demonstrate that \sys{} successfully watermarks layouts with an average of 1.85\% routed wirelength reduction for wirelength-driven ISPD'2015 and ISPD'2019 benchmarks and 7.48\% total negative slack improvement for timing-driven ICCAD'2015 benchmarks compared with the best-practicing prior art Row Parity~\cite{kahng2001constraint}, significantly reducing extra manufacturing costs from watermarking for the design houses. 
    \item  For the first time, we systematically categorize potential threats to the VLSI physical design watermarks into ghost, denial, and removal attacks. Extensive evaluations show \sys{} is resilient to all three types of attacks while maintaining over 90\% watermark extraction rates.  %\racheltodo{Are these 3 the only types of attacks we consider? The attacks should be defined in the introduction.}
    % \textcolor{blue}{Rachel: Include some numerical values here as you claim \sys{} to be better than row parity.}

\end{itemize}

\textbf{Paper Organization:} The rest of the paper is organized as follows:
Section~\ref{sec:background} provides the background on VLSI placement and VLSI watermarking.
Section~\ref{sec:goals} describes the problem formulation, including watermarking goals, threat model, and potential attacks.
%to our watermarks and challenges when performing watermarking.
Section~\ref{sec:method} introduces the proposed watermarking scheme \sys{}, by detailing global watermarking and detailed watermarking schemes and how these two techniques can be combined to strengthen the overall watermark.
Section~\ref{sec:exp} presents extensive experiments on various benchmark suites and demonstrates the effectiveness and robustness of \sys.
%baselines to demonstrate \sys's effectiveness.
Finally, Section~\ref{sec:conclusion} summarizes the work.
%The paper is concluded in .

%\ruisi{After routing and verification, the watermarks from the placement are infused into the final layout for fabrication.}
%\ruisi{To prove the ownership, the design house verifies the watermark by extracting the cells in the watermarked region and ensuring the cell positions match the intended watermark signature. }

 %\ruisi{ Extensive proof-of-concept evaluations on benchmark suites demonstrate that \sys{} improves the placement quality by 0.03\%, 0.93\%, and 0\% on ISPD 2005, ISPD 2015, and ISPD 2019, respectively, and improves the routing quality by 3.25\% and 0.04\% on  ISPD 2015, and ISPD 2019, respectively. } 



==> files_backup/1_intro_backup.tex <==

In the modern very-large-scale integrated circuit (VLSI) manufacturing supply chain, companies across multiple countries collaborate to design, fabricate, assemble, and verify integrated circuits (ICs)~\cite{liu2016vlsi,pawar2018risks,harrison2021malicious}.
The final product integrates intellectual property (IP) from various providers, e.g., design houses and fabricating houses, in the long supply chain. It is important to protect the IP~\cite{shamsi2019ip,knechtel2019protect,slpsk2023treehouse} at each supply chain step to avoid IP piracy attacks~\cite{guin2014counterfeit,yi2022impacts}, such as counterfeiting from malicious third parties.
The VLSI physical design consists of chip floorplanning, placement, and routing to bridge the logic design netlist to the GDSII layout for manufacturing. It optimizes the actual chip's physical layouts to reduce power consumption, area utilization, etc., saving chip producers millions of dollars in manufacturing costs. The layouts generated by the optimized algorithms during the physical design flow~\cite{lin2019dreamplace,mirhoseini2021graph,gu2020dreamplace} constitute an important IP.
However, they are prone to potential overbuilding and counterfeiting from untrusted third parties in the supply chain and are in need of protection. 



%%\racheltodo{Introduce the stages briefly before narrowing to placement stage in physical design. It would be good to include figure 1 for this.}
%The final product integrates IPs from various providers on the long IC supply chain, where the IP of each provider needs to be protected.  
%An important IP in the chip design flow is placement~\cite{lin2019dreamplace,mirhoseini2021graph,gu2020dreamplace}, which is the initial step for physical design, and significantly influences the power consumption, performance, and efficiency of design products.
%Several protection methods such as design obfuscation~\cite{narayanan2006limits,brakerski2014black,zhang2017dynamically,zhang2018chip,shamsi2019ip} and VLSI fingerprinting~\cite{caldwell1999effective,qu2000fingerprinting,prabhu2011extracting,stern2019emforced} have been introduced. These techniques are primarily tailored for routing or partition-based placement, thereby failing to provide proof of ownership for VLSI placements generated by modern analytical-based algorithms. 
%A promising set of solutions for safeguarding physical design IP is provided by embedding watermark signatures.
%Generally speaking, inserting watermarks in the VLSI layout presents several challenges.
%\ruisi{ }%The row parity watermarking~\cite{kahng2001constraint} does not account for the additional constraints during watermarking, resulting in diminished performance on certain benchmarks.

Watermarking~\cite{rathor2023hard,chen2023intellectual,tauhid2023survey} is a promising solution to protect physical design IP by embedding unique signatures. The signatures are based upon unique and confidential identifiers that are inconspicuous upon inspection and do not degrade the overall quality and performance of the IC.
To prove ownership, the design house verifies the watermark signature by extracting the embeddings from the IC layout. 

Nevertheless, inserting watermarks into the modern VLSI layouts is non-trivial. First, large-scale designs have dense standard cell connections, and slight perturbations of the cell location can degrade the overall performance. Second, modern ICs often have additional design constraints like fence regions and macros. Designing watermarking algorithms without considering these additional design constraints will diminish performance on certain benchmarks.
Finally, the watermarks should exhibit robustness against various potential attacks. For the first time, we have systematically categorized potential attacks into three distinct types based on the attack scenarios: \textit{Ghost Attacks}, where the adversary attempts to extract an alternative set of watermarks from the design, referred to as \textit{ghost watermarks}; \textit{Denial Attacks}, in which the adversary contends that the presence of watermarks is merely coincidental; and \textit{Removal Attacks}, where the objective of the adversary is to eliminate the embedded watermarks from the design.


Existing physical design watermarking schemes focus on placement and/or routing stages.
The placement watermarking-based approach named Row Parity~\cite{kahng2001constraint} inserts signatures by modifying the row index, where the row identifier of watermarked cells represents unique signatures via bit sequences. Though the placement watermarking scheme is simple to implement and guarantees $100\%$ watermark extraction rate, these techniques do not consider new constraints, such as fence regions and macros, that could lead to IC performance degradation. On the other hand, routing-based watermarks incorporate redundant wires to insert a signature, substantially increasing the overall wirelength cost~\cite{1510323}.
All these physical design watermarking schemes are susceptible to the ghost watermark attack, where adversaries with access to the design layout can implement another set of similar watermarks and claim ownership to the IC.


%} \ruisi{identifies regions and associated cells that undergo minimal performance deterioration after watermark embedding via a specialized scoring function.}


%The watermark region and cells within the region are added as a co-optimization term in global placement and legalization to enforce watermark insertion. %is introduced prior to the detailed placement to %

This paper devises \sys{}, a novel unified approach to safeguard layout IP by watermarking. It has no performance degradations after watermark insertion and is resilient to various potential attacks. 
\sys{} embeds signatures in the placement stage of the physical design process. The placement stage contains three submodules: global placement, legalization, and detailed placement. \sys's watermarks are infused in both global and detailed placement modules.  


The watermark insertion consists of two consecutive steps: 
(i) \textit{Global Watermarking} (GW) employs a specialized scoring scheme to identify watermarked cells on the watermarked region as GW signatures while ensuring minimal performance degradation.
(ii) Next, \textit{Detailed Watermarking} (DW)
inserts unique and confidential signatures hashed as bit sequences on top of the watermarked cells from GW. They are pervaded into the watermarked region by moving selected watermarked cells in the watermarked region along both the x- and y-axis.
The placement quality and the following GDSII layout quality for manufacturing are preserved by inserting watermarks on the regions that cause minimal performance degradation identified by the specialized scoring scheme from GW.
To verify the existence of signatures in the VLSI placement, \sys{} first extracts cells in the watermarked region and computes a watermark extraction rate for GW.
Then, the selected watermarked cell positions within the watermarked region are compared with the DW signatures to obtain a watermark extraction rate for DW. The two watermark extraction rates are computed collaboratively to intensify the watermark strength and fend off potential attacks. 


%The region extraction rate helps determine if a specific owner produces the placement. By calculating the cell extraction rate, the owner can include unique and confidential signatures, thereby augmenting the strength of the watermark.
%The subsequent detailed placement compensates for the performance degradation that originated from the watermark insertion, ultimately resulting in the watermarked placement with a minimal quality degradation.
%\racheltodo{I've commented out the details on which placement stage the watermarks are introduced. I did this because you haven't introduced placement or the different stages yet and to a reader without knowledge about placement it would not make sense.}

In brief, our contributions are  as follows:
\begin{itemize}
    \item We present \sys, a robust and unified watermarking scheme for the modern VLSI physical design pipeline, which does not degrade the layout quality while preserving 100\% watermark extraction rates.
    \item \sys{} employs a two-level watermarking approach to ensure minimal performance degradation. \textit{Global Watermarking} identifies the watermarked region of cells with minimal quality deterioration to insert watermarks, while \textit{Detailed Watermarking} perturbs the cells in the watermark region to inject unique signatures.
  %  \racheltodo{Here we only say that GW identifies region to watermark and DW inserts the signature. How does GW-only scheme watermark the cells in the selected region?}
    \item Extensive experiments on the ISPD'2005, ISPD'2015, and ISPD'2019 benchmark suites demonstrate that \sys{} successfully inserts watermarks without degrading estimated placement wirelength and routed wirelength. While the best-practicing baseline approach~\cite{kahng2001constraint} incurs an average of 0.44\% estimated placement wirelength and 1.56\% routed wirelength deterioration. 
    \item  For the first time, we systematically categorize potential threats to the VLSI physical design watermarks into ghost attacks, removal attacks, and denial attacks. Extensive experiments show \sys{} is resilient to all three types of attacks while maintaining over 90\% watermark extraction rates.  %\racheltodo{Are these 3 the only types of attacks we consider? The attacks should be defined in the introduction.}
    % \textcolor{blue}{Rachel: Include some numerical values here as you claim \sys{} to be better than row parity.}

\end{itemize}

\textbf{Paper Structure:} The rest of the paper is organized as follows:
Section~\ref{sec:background} provides the background on VLSI watermarking and VLSI placement.
Section~\ref{sec:goals} describes the watermarking scenario, challenges in watermarking, goals, and potential threats.
%to our watermarks and challenges when performing watermarking.
Section~\ref{sec:method} introduces the proposed watermarking scheme \sys{}, by detailing global placement watermarking and detailed placement watermarking schemes and how these two techniques can be combined to strengthen the overall watermark.
Section~\ref{sec:exp} details the extensive experiments on different benchmark suites and comparisons with existing watermark schemes.
%baselines to demonstrate \sys's effectiveness.
Finally, Section~\ref{sec:conclusion} summarizes the work.
%The paper is concluded in .

%\ruisi{After routing and verification, the watermarks from the placement are infused into the final layout for fabrication.}
%\ruisi{To prove the ownership, the design house verifies the watermark by extracting the cells in the watermarked region and ensuring the cell positions match the intended watermark signature. }

 %\ruisi{ Extensive proof-of-concept evaluations on benchmark suites demonstrate that \sys{} improves the placement quality by 0.03\%, 0.93\%, and 0\% on ISPD 2005, ISPD 2015, and ISPD 2019, respectively, and improves the routing quality by 3.25\% and 0.04\% on  ISPD 2015, and ISPD 2019, respectively. } 


==> files_backup/2_background.tex <==

\subsection{VLSI Placement}
%\textcolor{blue}{Rachel: Do we need this section? I think it would be better to have only one section on VLSI placement in which the first para could introduce VLSI design flow.}
The integrated circuit (IC) design implementation flow starts with design specifications that are converted to register transfer level (RTL) using a hardware description language (HDL).
As depicted in Figure~\ref{fig:physical_design}, the physical design process synthesizes the design HDL to generate a logic-level netlist comprising macros and standard cells from the technology library.
A floorplanning step determines regions and locations for the design's macros and the IO (input-output) ports.
This work considers macros locations to be fixed before placing all the standard cells.
Typically, the standard cells are placed during the placement stage, followed by routing all the design connectivity.
The routed design is verified to ensure manufacturability and generates the physical layout in GDSII format to send to the fabrication unit for manufacturing.
%The VLSI physical design is a crucial stage in integrated circuit (IC) design, wherein the logic representation of an IC is translated into a physical layout. The obtained physical layout details the placement of cells (including macros and standard cells) and the routing of interconnections between them. The process can be broadly delineated into five primary steps~\cite{otten2000challenges}: (i) floorplanning; (ii) placement; (iii) clock tree synthesis; (iv) routing; and (v) physical verification. Once these steps are successfully completed, photomasks for each layer are generated and forwarded to the fabrication facility for the manufacturing process.

 \begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/Physical_Design.pdf}
    \caption{%The VLSI physical design process. It bridges the input logic netlist to the GDSII layout for manufacturing.
    The VLSI physical design process. It generates the IC layout from a design RTL via synthesis, placement, and routing stages.}
    \label{fig:physical_design}
\end{figure} 

%Figure~\ref{fig:physical_design} depicts a simplified physical design process. Beginning with an input netlist, the chip floorplanning stage determines a rough arrangement of circuit cells on the chip canvas. Following this, the exact locations for standard cells are defined during the placement stage. After synthesizing the clock distribution network, the routing process defines the physical pathways for the electrical connections between cells. The culmination of this process is the physical verification step, which ascertains that the chip will function as intended during manufacturing.
%
%The \textcolor{red}{red cells} are denoted as macros, and the \textcolor{cyan}{blue cells} are standard cells. \href{https://lume.ufrgs.br/bitstream/handle/10183/197117/001096278.pdf?sequence=1}{in page 9 of this thesis}
%\subsection{VLSI Placement}
With fixed macro locations,
placement is an essential step in the physical design flow, which determines the locations of all the standard cells in the design~\cite{qiu2023progress,pawanekar2015nonlinear,agnesina2020vlsi,lin2021routability}. 
Placement significantly impacts the quality and efficiency of the subsequent stages, 
including routing and manufacturing.  Therefore, metrics, such as wirelength and timing, are considered in the placement formulation to improve the chip performance.
VLSI placement typically consists of three stages: Global Placement, Legalization, and Detailed Placement.

\subsubsection{Stage 1: Global Placement:} 
In the global placement stage, the placer aims to achieve roughly legal cell locations by distributing the cells across the chip area to minimize overlaps.
In addition to removing overlaps among the cells, the placer also targets other objectives, such as minimizing (i) wirelength and ensuring (ii) timing constraints are met.
%The first Global Placement stage distributes cells across the chip area to minimize a certain overall objective. Based on the objective functions to optimize, modern placers can be typically organized into two categories: (i) Nonlinear Global Placement and (ii) Timing-driven Global Placement. 

\noindent\textbf{Wirelength-driven Placement:}
%The overall placement can be formulated as the optimization objective in Equation~\ref{eqn:general_place}. It aims to minimize the estimated placement wirelength $W$ while ensuring minimal overlaps between the cells. Here, $(x,y)$ is the location of cells in the placement, $W(x,y)$ denotes the total wirelength of all cells in the design, and $D(x,y)$ is a density measure of the overlaps among the cells. Its constraint is set to below $\mathcal{D}$. 
%
%\begin{equation} \label{eqn:general_place}
%    min_{(x,y)} W(x,y) \ s.t.\  D(x,y) < \mathcal{D}
%\end{equation}
A wirelength-driven placer aims to minimize the overall wirelength $W$ while ensuring minimal cell overlap, as specified in Equation~\ref{eqn:general_place}~\cite{lin2019dreamplace,gu2020dreamplace, agnesina2020vlsi}.
\begin{equation} \label{eqn:general_place}
    min_{x,y} W(x,y) \ s.t.\  D(x,y) < \mathcal{D}
\end{equation}
where $(x,y)$ is the location of cells in the placement, and $W(x,y)$ denotes the total wirelength of all cells in the design. $D(x,y)$ is a density measure of the overlaps among the cells and it should be below $\mathcal{D}$.

\noindent\textbf{Timing-driven Placement:}
A timing-driven placer aims to optimize timing critical paths in the design while ensuring the overlaps among the cells are minimum~\cite{9774725}.
Given a timing endpoint $t$ (a primary output port or an input pin of memory element) with an arrival time of $t_{\mathrm{AT}}(t)$ and a required arrival time $t_{\mathrm{rat}}(p)$, the \textit{slack} of $t$ is calculated as follows,
\begin{equation} \label{eqn:timing_comp}
\begin{aligned}
slack(t) &= t_{\mathrm{RAT}}(t)-t_{\mathrm{AT}}(t) \\
TNS &= \sum_{t \in P_{\text {end }}} min(0,slack(t)) \\
WNS &= \min_{t \in P_{\text {end }}} slack(t) \\
\end{aligned}
\end{equation}
With the timing endpoints $P_{\text {end }}$ in the design, the total negative slack \textit{TNS} and the worst negative slack \textit{WNS} are computed as shown in Equation~\ref{eqn:timing_comp}.
A timing-driven placer optimizes either the \textit{WNS} or the \textit{TNS} to meet the timing constraint of the design.
%The overall timing-driven placement can be formulated as the optimization objective in Equation~\ref{eqn:timing_place}~\cite{9774725}.  Given a specific pin $p$ on the cell, its arrival time is defined as $t_{\mathrm{at}}(p)$ and its required arrival time is defined as $t_{\mathrm{rat}}(p)$. The slack of $p$ is defined as $s(p) = t_{\mathrm{rat}}(p)-t_{\mathrm{at}}(p)$. With the timing endpoints $P_{\text {end }}$ in the design, the total slack $S(\boldsymbol{x}, \boldsymbol{y})$ can either be calculated as total negative slack (TNS) where $S(\boldsymbol{x}, \boldsymbol{y}) = \sum_{t \in P_{\text {end }}, s(t)<0} s(t)$ or worst negative slack (WNS) where $S(\boldsymbol{x}, \boldsymbol{y}) = \min_{t \in P_{\text {end }}} s(t)$ depending on different design requirements. 
%The $D$ is the density measure of the bin $b \in B$, and $B$ is a set of grids in the design. \textcolor{red}{To Rachel: I borrowed the texts from DREAMPlace 4.0, but the $B$ variable here does not seem clear to me. Could you double check? Thanks. }
%
%\begin{equation} \label{eqn:timing_place}
%    max_{(x,y)} S(\boldsymbol{x}, \boldsymbol{y}) \ s.t.\ D_b(\boldsymbol{x}, \boldsymbol{y}) \leq d_t, \forall b \in B
%\end{equation}
%
\subsubsection{Stage 2: Legalization:}
The legalization stage eliminates any remaining overlaps among the cells and assigns legal locations that ensure row alignment while adhering to design constraints~\cite{spindler2008abacus,netto2021algorithm,yang2022mixed}.
The cells are legalized with minimal movement from their locations at the end of the global placement. During legalization, cells with multi-row heights are prioritized, undergoing legalization before the single-row height cells.

% During legalization, the multi-row height cells are legalized first before the single-row height cells.
%This second legalization stage~\cite{spindler2008abacus,netto2021algorithm,yang2022mixed} moves cells to guarantee they are positioned in legal locations and maintain the quality of the global placement, particularly in terms of wirelength and/or timing. The movements in legalization include eliminating overlaps, ensuring row alignment, adhering to specific design constraints, etc. 
%
\subsubsection{Stage 3: Detailed Placement:}
Finally, the detailed placement stage refines the legalized placement to improve design metrics such as wirelength or timing constraints~\cite{pan2005efficient,zhang2005global,chow2014cell}.
Some operations during detailed placement include (i) Swapping the positions of two cells to improve the objectives without causing legality or timing violations and (ii) Window-based approaches to find optimal cell locations within the specified region.
%The final stage detailed placement~\cite{pan2005efficient,zhang2005global,chow2014cell} further optimizes the overall placement quality by making small adjustments to the cell positions. It fine-tunes the placement for wirelength and/or timing optimizations. Some of the movements in detailed placement include (i) Swapping that exchanges the positions of two cells to improve objective optimization without causing legality or timing violations, (ii) Window-based detailed placement that optimizes the cell locations within a subregion of the design.
%
%
%To solve the optimization problem, researchers apply different methods like partitioning~\cite{dunlop1985procedure,tsay1991unified}, simulated annealing~\cite{sechen2012vlsi,chandy1996parallel}, and more recent analytical approaches~\cite{pawanekar2015nonlinear,lin2021routability,chen2012analytical}. 
%
\subsection{Watermarking in Chip Design}\label{subsec:wm_chip}
%\textcolor{red}{To Rachel: 1. Do you think we need to add other watermarking in the setting? 2. Could you double check if I missed any related work for the physical design wm?}

%\textcolor{blue}{Rachel: I found this \href{https://citeseerx.ist.psu.edu/document?repid=rep1&type=pdf&doi=0463206e28b320e747e6dc34f2cca8829f0c4005}{paper on digital watermarking} interesting.
%In addition to image, text and audio WM, I also found \href{https://www.sciencedirect.com/science/article/pii/S092523122101095X}{Neural Network WM}, as well as \href{https://www.inderscienceonline.com/doi/abs/10.1504/IJCAET.2020.103839}{video WM}.
%Here are some of the recent hardware or chip WM papers I found:
%(1) \href{https://ieeexplore.ieee.org/abstract/document/8839358}{Hardware Watermarking Using Polymorphic Inverter Designs Based On Reconfigurable Nanotechnologies},
%(2) \href{https://ieeexplore.ieee.org/abstract/document/9358262}{WaLo: Security Primitive Generator for RT-Level Logic Locking and Watermarking},
%(3) \href{https://ieeexplore.ieee.org/abstract/document/9983899}{ADWIL: A Zero-Overhead Analog Device Watermarking Using Inherent IP Features},
%(4) \href{https://ieeexplore.ieee.org/abstract/document/10174052}{PSC-Watermark: Power Side Channel Based IP Watermarking Using Clock Gates},
%(5) \href{https://ieeexplore.ieee.org/abstract/document/10226291}{Hard-Sign: A Hardware Watermarking Scheme Using Dated Handwritten Signature},
%(6) \href{https://dl.acm.org/doi/abs/10.1145/3526241.3530341}{Watermarked ReRAM: A Technique to Prevent Counterfeit Memory Chips},
%(7) \href{https://ieeexplore.ieee.org/abstract/document/9325223}{Hardware IP Protection Using Logic Encryption and Watermarking},
%(8) %\href{https://ieeexplore.ieee.org/abstract/document/10140093}{CAPEC: A Cellular Automata Guided FSM-based IP Authentication Scheme},
%(9) \href{https://ieeexplore.ieee.org/abstract/document/9284445}{On Database-Free Authentication of Microelectronic Components},
%(10) \href{https://arxiv.org/abs/2010.05209}{SIGNED: A Challenge-Response Based Interrogation Scheme for Simultaneous Watermarking and Trojan Detection}}

%\textcolor{blue}{This recent paper is on layout-level WM: \href{https://ieeexplore.ieee.org/abstract/document/9396208}{Identification of Integrated Circuits Based on Layout Layers Routing Information}}

%\textcolor{blue}{There's also a few recent book chapters on WM: \href{https://link.springer.com/chapter/10.1007/978-3-030-93274-9_5}{Watermarking for IP Protection}, 
%\href{https://link.springer.com/chapter/10.1007/978-3-031-19185-5_11}{Embedded Watermarks}}

%\textcolor{blue}{I think this recent paper would help with the story in introduction:
%\href{https://dl.acm.org/doi/abs/10.1145/3453688.3461758?casa_token=xTsnAvd4qY4AAAAA:C2AvlnqE-Ngu7SSJCVBJPp_cNKW3bP_ziPAuKTJCvNxygZh-r9eoPEBC28S4QzKkeETg0V_BQUTRNQ}{The Curious Case of Trusted IC Provisioning in Untrusted Testing Facilities}}

%\textcolor{blue}{Some older papers on IC WM - Some are layout WM:
%(1) \href{https://ieeexplore.ieee.org/abstract/document/694985}{Hierarchical watermarking in IC design}
%(2) \href{https://www.proquest.com/docview/1624973929/fulltextPDF/E73F762962D34E64PQ/1?accountid=7118}{Watermarking ICs for IP protection}
%(3) our baseline \href{https://ieeexplore.ieee.org/abstract/document/952740}{Constraint-based watermarking techniques for design IP protection}
%(4) \href{https://ieeexplore.ieee.org/document/5513117}{Side-channel based watermarks for integrated circuits}
%(5) \href{https://digital-library.theiet.org/content/journals/10.1049/el_20030874}{Watermarking for intellectual property protection}
%}

%Watermarking is a prevalent technique in various domains, including image~\cite{zhong2020automated,neekhara2022facesigns}, text~\cite{ahvanooey2020anitw,hilal2022hybrid}, and audio processing~\cite{zhang2022robust,salah2021fourier}, allowing creators to assert their intellectual property (IP) rights without compromising product quality. 
Design houses leverage watermarking in the long chip supply chain to enhance IP rights protection and detect unauthorized usages or replications. Those watermarks are typically inserted in the logic design or physical design level. 

\subsubsection{Logic Design Watermarking:} 
The watermarking at the logic design level focuses on safeguarding the Register Transfer Level (RTL) or netlist ownership. Designers embed unique signatures into the RTL or netlist that do not impact the core functionality and are invisible upon adversaries' inspection. The signature insertion can be categorized as follows: (i) modifying the finite state machine (FSM) to add additional inputs or unused components as watermarks~\cite{5938070,divyanshu2023fsm}; (ii) adding additional power components as side-channel signatures~\cite{becker2010side,das2023psc}; and (iii) introducing unique triggers during netlist design that induces the variant function when the triggers are detected~\cite{8764416}. 

%The objective of netlist-level watermarking is to protect the intelligent property of the logic design process.
%By embedding the signatures into the circuit cell connection, watermarking helps IP owners claim RTL or netlist ownership. Designers can add specific patterns of gates or additional components into the netlist that doesn't affect the chip's functionality but are identifiable upon inspection. 

More recent work introduced logic locking to add additional logic gates and circuits 
 that alter the functionality of the original design when the incorrect key is applied~\cite{sengupta2020truly,kamali2022advances}; obfuscation to adding dummy logic gates or additional circuit connections to make the logic design appear differently from the original one~\cite{santikellur2021hardware,bagul2023hardware}. These techniques are orthogonal to the logic design watermarking, which can be combined to establish more robust IP protection frameworks.

\subsubsection{Physical Design Watermarking:} 
It is beneficial to watermark at the physical design stage instead of the logic design for the following reasons.
(i) Adding additional watermarks into the logic design needs to consider physical design criteria like timing to maintain chip quality. However, watermarking after these constraints have been optimized at the physical design stage reduces those burdens. (ii) In logic design, if the logic circuits are not performing correctly after watermark insertion, designers need to revisit the RTL design in the previous stage. Physical watermarking, however, does not modify the circuits' functionalities and only focuses on how cells are placed on the chip canvas.

%\rachel{IC watermarking is done at different stages - logic design and Physical design.}
%\racheltodo{Include few sentences on logic design watermark at RTL and others not physical design.}
%IC watermarking can be done at different stages, including logic and physical designs. The logic design watermarks are at the RTL or netlist level, whereas 
The physical design watermarking inserts signatures on the IC layout during the placement or routing stages. In the placement stage, row parity~\cite{kahng2001constraint} enforces some of the cells to be on odd or even rows, and their row indexes are represented as watermarking signatures. However, the cell movements do not consider other design constraints in modern VLSI benchmarks like fence regions. It would introduce increments in the wirelength or timing metric in the final layout. 
Guangyu Sun~\textit{et.al}~\cite{1613214} proposed to add redundant cells in the placement stage as unique signatures. However, the redundant cells can be easily removed if the adversary can access or reverse-engineering the layout~\cite{9300272}. 
In the routing stage~\cite{1510323},  Nie, T~\textit{et.al}~\cite{1510323} proposed to enforce wires under certain constraints are bent to embed as watermarks. The wire bends will subsequentially increase the routed wirelength in the final layout and introduce extra costs for manufacturing. Besides, deciding which wire to bend under constraints becomes computationally heavy as the size of the nets increases.

%Physical design watermarking protects the intelligent property of the layout generated in the physical design process.
%\ruisi{Despite these drawbacks, when verifying ownership at the layout level, watermarking at the physical design stage instead of the logic design stage exhibits the following benefits: (i) Adding additional watermarks into the logic design needs to consider physical design criteria like timing to maintain chip quality. However, watermarking after these constraints have been optimized at the physical design stage reduces those burdens. (ii) In logic design, if the logic circuits are not performing correctly after watermark insertion, designers need to revisit the RTL design in the previous stage. Physical watermarking, however, does not modify the circuits' functionalities and only focuses on how cells are placement on the chip canvas.}


%However, existing physical design watermarking techniques encounter several drawbacks. First, the row parity-based algorithm faces significant quality deterioration when accommodating additional constraints (e.g., fence regions) in the placement stage. Secondly, watermark wire selection during the routing stage requires specific constraints. Determining wires under these constraints becomes computationally heavy as the size of the nets increases. 

In this work, we introduce \sys—a robust and effective watermarking framework tailored for modern, large-scale VLSI physical designs.

%watermarking at the physical design level exhibits several benefits compared with logic-level watermarking: (i) watermarking at the logic level 






%1. Include extra information on why physical design wm is better than logic design wm. (motivation) (II) adding wm logic design needs to consider the quality of chip like timing; but physical design is easier to wm. Physical design reduces the effort of redesigning the logic level information if the wm is inserted, which is planned early in the RTL design.  

%The objective of layout-level watermarking is to protect the intelligent property of the physical design process. Previous work achieves this by enforcing the placement of specific cells or adding additional wires in the routing stage. However, these works tend to introduce additional wirelength into the design and thus compromise the physical design quality. 



%\ruisi{including layout, placement or routing.}
%, and post-placement level via the addition of incremental routings~\cite{1510323}. 
%\textit{Kahng et al.} proposed a comprehensive watermarking protocol for VLSI design that encompasses each level~\cite{kahng2001constraint}. However, this watermarking methodology falls short in accommodating modern VLSI placement algorithms, in which the total cell count can escalate into the millions, and multiple constraints, such as fence regions or macros, need to be taken into account. Several subsequent work have proposed the insertion at the physical level using buffers~\cite{1613214}, at the post-placement level through the addition of incremental routings~\cite{1510323}, or by incorporating dummy fillers~\cite{saha2014watermarking}.

%
%Equation~\eqref{eqn:general_place} can be relaxed as an unconstrained optimization problem as,
%\begin{equation} \label{eqn:place}
%    \min_{x,y} f(x,y) = \min \bigg( \sum_{e \in E} W_e(x,y) + \lambda D(x,y) \bigg),
%\end{equation}
%where $W_e(x,y)$ represents the wirelength of design net $e \in E$ and $\lambda$ is the Lagrangian multiplier for the density term $D(x,y)$.

%Half-perimeter wirelength (HPWL) is generally used to estimate the overall wirelength and depends on the bounding box of all the pins connected to a net $e$,
%\begin{equation} %\label{eqn:HPWL}
%    W(x,y) = \sum_{e \in E} \Big( \max_{i,j \in E} |x_i - x_j| + \max_{i,j \in E} |y_i - y_j| \Big) .
%\end{equation}

==> files_backup/3_threat.tex <==
In this section, we outline the goal of \sys, along with introducing the threat models and potential attacks when integrating watermarked layout into the supply chain. %Next, we highlight several challenges that \sys{} confronts during the watermark insertion process.

\subsection{Watermarking Goals}

\sys{} establishes ownership proof for the VLSI physical design by inserting watermarks into the placement stage, thereby authenticating the IP for the final layout. Figure~\ref{fig:scenario} depicts a typical scenario within the supply chain. IC design companies employ highly customized and optimized placement and routing algorithms to enhance the physical design quality. Then, these layouts from the physical design stage are watermarked and sent to the fabrication company for manufacturing. The manufactured ICs are verified for their functionalities in the test company. 


\begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/vsli_wm_scenario.pdf}
     \caption{IC layout watermark scenario in the supply chain. The design company watermarks the IC Layout before sending it for manufacturing and testing in the supply chain.}
    \label{fig:scenario}
\end{figure}

In the physical design stage, large IC design companies invest huge efforts to identify and fine-tune constraints tailored for cell placement and net routing optimization. The optimization and customization are infused into different levels of the final layout, including (but not limited to) blocks and cells, to boost IC performance and reduce manufacturing expenses. The algorithm optimizations and customizations of the physical design process constitute invaluable intellectual property, emphasizing the need to safeguard it. We present \sys{} as a watermarking framework to protect intellectual property in physical design. It is designed with three fundamental criteria as follows:

\noindent\textbf{Effectiveness:} The embedded watermarks are readily extractable, ensuring the layout's ownership identification.

\noindent\textbf{Quality Preservation:} The insertion of watermarks does not compromise the layout quality. 

\noindent\textbf{Resilience:} The watermarking framework exhibits robustness, ensuring the watermarks can withstand various potential attacks within the supply chain.


\subsection{Threat Model}

We consider the general supply chain scenario where an IC design company $D$ possesses a customized and optimized layout solution, denoted as $L_D$, along with a set of watermarks, referred to as $W_D$. The design company employs $W_D$ to help prove the ownership of $L_D$. The adversary $A$ aims to stop $D$ from claiming its ownership by executing different attacks.

\noindent\textbf{Adversary’s Locations:} We consider the adversary $A$ to be in the fabrication or test company that has access to the layouts produced by the design company. %Those companies are untrusted because building confidential breaches can be extremely costly to IP vendors and IC design companies. 


\noindent\textbf{Attack Scenario:}  Adversary $A$ in the fabrication company overbuilds the ICs using the layouts $L_D$ from the design company $D$. They make profits by selling those unlicensed and unintended ICs to the market.

%We introduce two attack scenarios, namely \textit{Counterfeiting} and \textit{Overbuilding} as follows:

%\begin{itemize}
%\item \textbf{Counterfeiting:} Adversary $A$ in the fabrication company make profit by selling counterfeited layout $L_A$. They claim the design is from design company $D$ with counterfeited watermark $W_A$ as proof. 
 
%\item \textbf{Overbuilding:}
%\end{itemize}


\noindent\textbf{Adversary’s Capacities:} The optimizations and customizations for better IC performance metrics are embedded at various levels of the layout. Therefore, it becomes infeasible for the adversary $A$ to extract those constraints from the layout and independently execute the physical design using open-source tools. The only way for the adversary to steal intelligent property is to overbuild the watermarked layout from the design companies. 

\begin{itemize}
    \item The adversary $A$ has access to the layout solutions. But he does not know how those modules are customized and optimized. 
    \item The adversary $A$ has access to open-source physical design tools to overbuild the watermark. He also knows the general algorithms to watermark the layout. However, the random seeds, signatures, and insertion parameters are beyond his reach.
    \item The overbuilt layout performance degradation, measured by total wirelength or timing metrics, should not exceed 0.5\% of the original layout from the design company. Otherwise, the extra effort the design company spent on optimizing the IC layout is compromised.
\end{itemize}

\textbf{Adversary’s Objective:} Adversary $A$'s objective is to prevent design company $D$ from establishing its layout ownership claims by executing different attacks. 

\subsection{Potential Attacks}\label{sec:potential_attacks}

\noindent\textbf{Attack 1: Ghost Attack}~\cite{liu2016vlsi} Adversary $A$ aims claim his ownership of layout $L_D$ by extracting another set of ghost watermarks $W_A$ from $L_D$, and claim the actual watermark in the IC is $W_A$ instead of $W_D$.


\noindent\textbf{Attack 2: Denial Attack}~\cite{yuan2006vlsi} Adversary $A$ proposes that the layout solution was generated using open-sourced algorithms and suggests that the presence of the watermark $W_D$ is coincidental. %By employing this strategy, $A$ attempts to deny $D$'s ownership rights by asserting that the watermark's presence in the layout is not deliberate.% \ruisi{Cite a reference here if possible - a paper or article or even news on such attacks}

\noindent\textbf{Attack 3: Removal Attack}~\cite{liu2016vlsi}  Adversary $A$ intentionally alters cells positions within the layout solution $L_D$ to remove the watermark $W_D$ added by the design company. %This attack aims to invalidate $D$'s ownership claim by tampering with the watermarks. %\ruisi{Cite a reference here if possible - a paper or article or even news on such attacks} 




==> files_backup/3_threat_backup.tex <==
%\ruisi{It would be nice to include a few lines describing what to expect in this section. The tile only says Goals and Threats, but then there is also a subsecion on Challenges. Adding a few sentences at the start would help the reader.}

%\todo{1. clearly state in 3.1 that we are protecting the customized \& optimized placement tools 2. Restate the attackers' capacities. }

In this section, we first delineate the goal of \sys, along with threat models \sys{} encounters when integrating its placement watermarks into the supply chain. Next, we highlight several challenges that \sys{} confronts during the watermark insertion process.

\subsection{Placement Watermarking Goals}
In this paper, we provide ownership proof for VLSI placement solutions in the supply chain. While existing works have explored the insertion of unique signatures at routing or partition-based placement, we are the first to address IP protection for modern analytical-based VLSI placements.

Figure~\ref{fig:scenario} illustrates a typical scenario within the supply chain. Chip design companies employ customized and optimized placement algorithms to enhance the design quality and send them to downstream fabricate and test companies for manufacturing. Those improved placement algorithms are designed at different levels of the VLSI placement, such as block, cell, and hierarchical levels, aiming to boost chip performance, reduce power consumption, and improve area efficiency. It usually takes weeks or months for researchers and engineers in these large chip design companies to work together and find such chip cell placement constraints~\cite{}. 
\begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/scenario.pdf}
     \caption{Watermark Scenario for \sys.}
    \label{fig:scenario}
\end{figure}

Such placement details are easily to be accessed by third 

We argue that optimized and customized placement solutions in the VLSI design loop constitute important intelligent property and are at risk of being attacked under many scenarios, as mentioned previously. However, there is a lack of such fine-grained IP licensing in the design workflow to provide ownership proof for the placement design team without sharing the routing details subsequently. 
To address this problem and provide ownership proof, we build an innovative unified watermarking scheme named \sys{} to safeguard the optimized VLSI placement algorithm in the supply chain.




\subsection{Threat Model}
We consider the general scenario where a chip designer \textit{Alice} possesses a customized and optimized placement solution, denoted as $P$, along with a set of watermarks, referred to as $W_A$, which she intends to employ as evidence of ownership. The adversary \textit{Bob} aims to stop \textit{Alice} from claiming her ownership.


\textbf{Attack Scenario:} We introduce two general attack scenarios, namely \textit{Overbuilding} and \textit{Counterfeiting}, in the chip supply chain and showcase the VLSI placement solutions are prone to be attacked. 


\begin{itemize}
    \item  Counterfeiting: In this setting, the untrusted foundry / testing facility uses low-quality placement and subsequent routing for fabrication. They claim the design company produces the placements by providing their counterfeited watermarks.
    \item Overbuilding: In this setting, given the layout from the chip companies, the untrusted foundry / testing facility aims to overbuild the chip by changing the placement design slightly to remove watermarks $W_A$. They manufacture and sell those chips to the black market for additional profits. 
\end{itemize}

\textbf{Adversary’s Locations:} We consider the adversary \textit{Bob} to be in the later stage of the supply chain. He can be an untrusted foundry or testing facility. \textit{Bob} has access to the final placement $P$ and has access to open-source tools to modify $P$. However, \textit{Bob} does not have access to the placement modules aiming to enhance placement quality or customize placement criteria. 

\textbf{Adversary’s Capacities:} In this threat model, the placement constraints are spread among the VLSI placement solutions at different levels. Therefore, it is impossible for the adversary to extract those constraints and get their solutions by running on open-sourced placement tools. The only way for the adversary to steal intelligent property is to overbuild or counterfeit the placement watermarks from the design companies. 

\begin{itemize}
    \item The adversary \textit{Bob} has access to the VLSI placement solutions. But he does not know which modules are been customized and optimized. Nor does he know how most of the constraints are designed.
    \item The adversary \textit{Bob} has access to open-source VLSI placement tools to overbuild or counterfeit the watermark. He also knows the general algorithms to watermark the placement but cannot access the random seeds / signatures and insertion parameters.
    \item After the watermark is overbuilt or counterfeited, the placement should still be usable. It means the VLSI placement performance degradation, measured by Half-Perimeter Wirelength (HPWL), should not exceed 0.5\% of the placement from the design company. Otherwise, the manufacturing process will introduce several million dollars in extra costs for the adversaries. 
\end{itemize}


\textbf{Adversary’s Objectives:} \textit{Bob}'s objective is to prevent \textit{Alice} from establishing her placement ownership claims by executing the different attacks in Sec.~\ref{sec:potential_attacks}. 




\subsection{Potential Attacks}\label{sec:potential_attacks}

\noindent\textbf{Attack 1: Ghost Attack}~\cite{liu2016vlsi} With the placement solution $P$, \textit{Bob} extracts an alternative set of watermarks, denoted as $W_B$, from the placement. By falsely asserting that the injected watermark within the placement is $W_B$, \textit{Bob} aims to hinder \textit{Alice} from asserting her ownership by disputing the authenticity of the actual watermark $W_A$. %\ruisi{Cite a reference here if possible - a paper or article or even news on such attacks}

\noindent\textbf{Attack 2: Removal Attack}~\cite{liu2016vlsi} \textit{Bob} intentionally perturbs cells within the placement $P$ to disrupt the watermark $W_A$ added by \textit{Alice}. This attack aims to invalidate \textit{Alice}'s ownership claim by compromising the integrity of the watermark embedded in the placement. %\ruisi{Cite a reference here if possible - a paper or article or even news on such attacks}

\noindent\textbf{Attack 3: Denial Attack}~\cite{yuan2006vlsi}  \textit{Bob} proposes that the placement solution was exclusively generated using open-sourced algorithms, suggesting that any presence of the watermark $W_A$ is coincidental. By employing this strategy, \textit{Bob} attempts to deny \textit{Alice}'s ownership rights by asserting that the watermark's inclusion in the placement is not a deliberate act.% \ruisi{Cite a reference here if possible - a paper or article or even news on such attacks}
 


%\ruisi{cite the paper. Also use a common term to specify the baseline. Use either 'row parity' or 'row-parity' etc, but be consistent}
%The watermarks should be unique such that ghost attack and denial attack that aims to override watermarks on current placement fails. The previous row parity approach falls short in this aspect, as it randomly selects standard cells, making it easier for adversaries to extract another set of watermarks and override the placement's original watermarks.

 
\subsection{Challenges}

To effectively defend the threat model without degrading overall placement quality, we identify three challenges:

\noindent\textbf{Challenge 1: Dense Connections} Due to dense interconnections within the placement cells, randomly changing cell positions without considering the overall distribution will result in huge performance degradations. Thus, developing a watermarking approach that considers the dense nature of cell connections to minimize negative impacts on the placement quality is crucial.

\noindent\textbf{Challenge 2: Design Constraints} Current placements benchmark suites incorporate additional design constraints, such as fence regions, into the placement process. However, the previous row parity based approach~\cite{kahng2001constraint} resulted in placement quality degradation when adding those constraints into the design loop.
%The resulting watermarking placement exhibited substantial degradation compared to non-watermarked solutions. 
A more comprehensive approach is required to address these additional constraints while embedding watermarks effectively.


\noindent\textbf{Challenges 3: Confidentiality} The watermark within the placement must be confidential to prevent ghost attacks on the watermarked solutions. In the row parity approach~\cite{kahng2001constraint}, adversaries can easily extract another set of watermark cells and their row identifiers from the placement as ghost watermarks. It is essential to devise a watermarking method that ensures the confidentiality of the watermark, thereby enhancing its security against such attacks.

==> files_backup/4_method.tex <==
%The watermarking pipeline is illustrated in Figure~\ref{fig:overview}. \sys is a unified watermarking scheme consisting of two steps: \textit{Global Watermarking} and \textit{Detailed Watermarking}. The objective of the \textit{Global Watermarking} is to identify regions where the inclusion of a small fence region, along with the watermarked cells within that region, results in minimal overall performance degradation. Following \textit{Global Watermarking}, the \textit{Detailed Watermarking} focuses on perturbing cells specifically within the identified region to inject unique signatures. This is achieved by perturbing cells with available space to move along the x and y axis. 


%\todo{1. restate the detailed watermark is actually strengthen the watermark}

This section presents the proposed layout watermarking \sys{}, a two-level scheme that inserts watermarks at multiple stages during VLSI placement. In Section~\ref{sec:GW}, we introduce a \textit{Global Watermarking} method.  Next, we propose an independent embedding of the watermark signatures as \textit{Detailed Watermarking} in Section~\ref{sec:DW}. These two watermarking methods can each be used independently for IP protection, and as such, we provide comprehensive evaluations of their quality and resiliency to attacks. \sys{} in Section~\ref{sec:sys} is a hybrid methodology that combines both \textit{Global} and \textit{Detailed Watermarking} to take advantage of the best properties of independent global and detailed watermarking techniques. 

%\textcolor{red}{Given a layout solution with optimized constraints to enhance power-performance-area (PPA) metrics, design companies intend to protect their IP by watermarking the layout. }

\subsection{\textit{Global Watermarking} (GW)} \label{sec:GW}
\textit{Global Watermarking} embeds watermarks during the global placement stage. The watermarks, including a pre-defined watermarked region and associated watermarked cells, are embedded as a co-optimization term during global placement. It ensures only those associated watermarked cells are placed in the watermarked region. 

\subsubsection{\textbf{GW Watermark Selection}} 

Given the original, optimized placement denoting the position of all cells as $P_{ori}$, we utilize a sliding window approach that traverses the placement with a fixed stride in search of potential regions to insert as watermarks.
An ideal watermarked region should meet three criteria: (i) the number of cells within the region should be sufficient to insert the required number of signature bits; (ii) the total area of cells within the region should be small, thereby providing ample space for watermarked cells to maneuver; and (iii) for cells on the region boundary, their overlapping area within the region should be minimized, ensuring that cell displacement from the watermarked region insertion does not significantly impair performance. These requirements are formulated into an evaluation function $f$, as illustrated in Equation~\ref{eq:score}. It evaluates each region of the chip canvas where cells have been placed according to $P_{ori}$. Note that obtaining $P_{ori}$ with pre-defined physical design optimization and customization is not time-consuming. The most time-intensive aspect of physical design is finding those optimization constraints. 

%the dominant time-consuming part in physical design lies in identifying optimized constraints to be incorporated into the physical design algorithm rather than the execution of the algorithm itself.
 
\begin{equation}
\label{eq:score}
    f = \alpha \frac{|N_w|}{|N_c|} + \beta \frac{S_{cell}}{S} + \gamma \frac{S_{overlap}}{S}
\end{equation}

\begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/global_wm.pdf}
     \caption{Global watermarking pipeline. The stride is set to the same as the sliding window size.
     %Global watermarking pipeline. For ease of explanation, we set the stride to be the same as the sliding window size. However, the stride is much smaller than the widow size in the experiment. 
     }
    \label{fig:global}
\end{figure}


Here, $|N_w|$ is the length of the signature sequences to be inserted and $N_c$ is the cells within the region.   
$S_{cell}$ is the total cell size area of $N_c$, $S$ is the total region area, and $S_{overlap}$ is the total area of overlapping cells $N_o$  within the region.  The scoring function is balanced by adjusting the weights $\alpha$, $ \beta$, $\gamma$, where  $\alpha, \beta, \gamma \in [0,1]$.  

For regions that overlap with macros or other fence regions and any region where $|N_c| < |N_w|$, it yields higher evaluation scores, rendering the regions not suitable for inserting GW watermarks. These region scores are close to 1.0, as denoted in red in Figure~\ref{fig:global}.
The region with the minimum score is chosen as our target watermarked region $K_w$, and the set of watermarked cells within the region is denoted as $C_w$. 


\subsubsection{GW Watermark Insertion}
The watermarked region $K_w$ containing watermarked cells $C_w$ is formulated as an additional region constraint in the placement objective. It enforces the watermarked cells $C_w$ to be in the watermarked region $K_w$ and other cells to be out of $K_w$.
For a design with $K$ fence regions, the placement formulation to include region constraints is specified in Equation~\ref{eq:multiregion}~\cite{gu2020dreamplace}.
$W$ is the wirelength term and $D$ is the cell density term with density multiplier $\lambda$. $v$ denotes the $(x,y)$ location of cell and $e\in E$ is the design net.
The watermarked region is added as an additional region constraint $K+1 = K_w$ with watermarked cells $C_w$ to obtain a watermarked placement $P_w$.
\begin{equation}
\label{eq:multiregion}
\begin{array}{ll}
\min _v & \sum_{e \in E} W(e ; v)+\lambda D(v), \\
\text { s.t. } & v_k=\left(x_k, y_k\right) \in r_k, \quad k=0, \cdots, K, K+1,
\end{array}
\end{equation}

\noindent\textbf{GW Watermark Strength:} The selection of the watermarked region and watermarked cells is random because different values of the parameter settings $\alpha$, $\beta$, $\gamma$, and sliding window sizes result in different watermarks. The p-value denoted as $P_c$ in statistical Null Hypothesis test~\cite{berger1987testing} measures the probability of a solution carrying the watermark purely by coincidence.
A smaller $P_c$ means a stronger watermark signature insertion. 
The probability that an overlapping cell in $N_o$ is out of the watermarked region $K_w$ is denoted as $p$, and the probability of the overlapping cell to be in or overlap $K_w$ is $1-p$. 
If no watermark is inserted, the $N_o$ cells should overlap with the watermark region. We measure the probability that $x$ or more cells match the watermarking condition, that is, they are out of the watermarked region, as the probability of $P_c$ in Equation~\ref{eq:gp_strength}. $\mathbf{C}$ is the number of combinations of selecting $i$ elements from $|N_o|$ distinct elements.
%We can get the probability of $P_c$ that $x$ or more overlapping cells are out of the region  $K_w$ from Equation~\ref{eq:gp_strength}. 
The placement algorithms tend to place cells more compactly, which means the probability of a cell being away from its original place $p < 0.5$. In Equation~\ref{eq:gp_strength}, $P_c$ is an increasing function of $p$ when $p\in[0, 0.5]$. For simplicity of computation, we set $p=0.5$ as an upper bound for $P_c$. In reality, $P_c$ is even smaller because the position and size of the watermarked region are not revealed to the adversary, and it introduces more randomness to strengthen $P_c$. 
%\textcolor{red}{To Rachel: Could you double-check if the watermark strength formulation is clear?}

\begin{equation}
\label{eq:gp_strength}
\begin{array}{ll}
P_c = \sum_{i=x}^{|N_o|}\left(\mathbf{C}(|N_o|, i) \cdot(1-p)^{|N_o|-i} \cdot(p)^i\right) 
\end{array}
\end{equation}

\subsubsection{GW Watermark Extraction}
%\textcolor{red}{To Rachel: I think we need to mention how to reverse engineer from the layout/chip to cell positions here. But is there any related work I can cite?}
%\rachel{You can cite this \href{https://ieeexplore.ieee.org/abstract/document/9300272}{work}. It is possible to easily get the locations of all the standard cells.}

Reverse engineering approaches like ReGDS~\cite{9300272} can extract logic netlist and all standard cell locations from an IC layout in GDSII format.
The design owner asserts ownership by employing the watermarked region $K_w$ to extract cells $C_w^\prime$ within the region and comparing these with the watermarked cells $C_{w}$ and non-watermarked cells $C_{wo}$. The extraction rate of the watermark, denoted as $WER_{GW}$, is calculated in Equation~\ref{eq:gw_wer}.

\begin{equation}
\label{eq:gw_wer}
\begin{array}{ll}
\%WER_{GW} = 100\times\frac{ |(C_w^\prime \cap C_{w}) - (C_w^\prime \cap C_{wo})|}{|C_{w}|}
\end{array}
\end{equation}


\subsection{\textit{Detailed Watermarking} (DW)}\label{sec:DW}
In \textit{Detailed Watermarking}, the watermarked cells are embedded by moving them slightly along the x- or y-axis after legalization. The follow-up detailed placement compensates for the performance degradation from the watermark insertion. 

\subsubsection{DW Watermark Selection}
The \textit{Detailed Watermarking} moves cells along the x- or y-axis to insert watermarks into the design. Randomly selecting watermarked cells and moving them without considering the dense interconnection could lead to significant performance degradation. To avoid this, \textit{Detailed Watermarking} only selects and moves cells with sufficient room to accommodate the watermark as shown in Figure~\ref{fig:detail_wm}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/detail_wm.pdf}
     \caption{Detailed watermarking pipeline. \textcolor{purple}{Candidate cells} available to move are marked in purple, \textcolor{orange}{Watermarked cells} are marked in orange}
    \label{fig:detail_wm}
    \vspace{-0.5cm}
\end{figure}


Algorithm~\ref{alg:select_cells} outlines how \textit{Detailed Watermarking} identifies cells with enough space for movement and subsequently inserts watermarks. It starts by comparing the positions of cells within each row and identifying the cell indices that can move along the x-axis. Then, the algorithm compares cells across neighboring rows to determine if they can be moved up or down. The cells, $C_x$ with room along the x-axis and $C_y$ with room along the y-axis are identified as candidate cells for watermarking. $D_x$ and $D_y$ are associated with these candidate cells to retain a record of their movement directions and distances. The units of distance in $D_x$ and $D_y$ are set as absolute values $|d_x|$ and $|d_y|$, respectively. For movement along the x-axis, if the cell shifts to the right, the distance added to $D_x$ is positive, i.e., $|d_x|$. Conversely, if the cell moves to the left, the added distance is negative, i.e., $-|d_x|$. Similarly, $|d_y|$ is added to $D_y$ if the cell ascends to the above row, and $-|d_y|$ if it descends to the below row.

\begin{algorithm}[ht]
\caption{DW Watermark Selection and Insertion}
\label{alg:select_cells}
\small
\begin{algorithmic}[1]
    \REQUIRE Legalized placement \( (X_{lg}, Y_{lg}) \), Signature \( B_N \), Unit distance $|d_x|$ and $|d_y|$
    \ENSURE Watermarked cells \( C_{wm} \), Placement \((X_{wm}, Y_{wm})\)

    \STATE Initialize empty sets \( C_x, C_y, D_x, D_y \)
  %  \STATE Identify candidate watermarked cells by examining their room to move along the x and y-axis.
    
    \FOR{\( r = 0 \) to total\_num\_rows}
        %\STATE \( C_r = \text{get\_cells\_in\_row}(r) \)
        %\FOR{\( c \) in \( C_r \)}
        \FOR{\( c \) in \( \text{cells\_in\_row}(r) \)}
            %\IF{\( \text{is\_movable\_x}(c, C_r) \)}
            \IF{\( \text{is\_movable\_x}(c) \)}
                \STATE Append \( c \) to \( C_x \)
                \STATE \( s = \text{get\_direction\_x}(c) \)  \DontPrintSemicolon \ \ \tcp{left: -1; right: 1} 
                \STATE Add \( (s \times |d_x|) \) to \( D_x \)
            \ENDIF
            %\IF{\( \text{is\_movable\_y}(c, C_r) \)}
            \IF{\( \text{is\_movable\_y}(c) \)}
                \STATE Add \( c \) to \( C_y \)
                \STATE \( s = \text{get\_direction\_y}(c) \)  \DontPrintSemicolon \ \ \tcp{down: -1; up: 1} 
                \STATE Add \( (s \times |d_y|) \) to \( D_y \)
            \ENDIF
        \ENDFOR
    \ENDFOR
    
    \STATE Random shuffle \( C_x \) and \( C_y \)
    \STATE \( X_{itr}, Y_{itr} = X_{lg}, Y_{lg} \)
    
    \FOR{\( i = 0 \) to \( |B_N| \)}
        \IF{\( B_N[i] == 1 \)}
            \STATE \( c_i = \text{random\_choose}(C_x) \)  \DontPrintSemicolon \ \ \tcp{no replacement}
            \STATE \( X_{itr}[c_i] = X_{lg}[c_i] + D_x[c_i] \)
        \ELSE
            \STATE \( c_i = \text{random\_choose}(C_y) \) \DontPrintSemicolon \ \ \tcp{no replacement}
            \STATE \( Y_{itr}[c_i] = Y_{lg}[c_i] + D_y[c_i] \)
        \ENDIF
        \STATE Add \( c_i \) to \( C_{wm} \)
    \ENDFOR
    
    \STATE \( X_{wm}, Y_{wm} = \textit{detailed\_placement}(X_{itr}, Y_{itr}) \)
    \STATE \textbf{return} \( C_{wm}, X_{wm}, Y_{wm} \)
    
\end{algorithmic}
\end{algorithm}

\vspace{-0.3cm}

%The probability $P_c$ of a solution carrying the watermark purely by coincidence can be used to measure the strength of our algorithm. The probability of $x$ or fewer cells in $N_o$ to be in $K_w$ is $p$  and out of $K_w$ to be $1-p$, we can get  $P_c$ from Equation~\ref{eq:gp_strength}. Due to the nature of placement algorithms, they tend to place cells more compactly, which means the probability $p > 0.5$. Besides, $P_c$ is a decreasing function of $p$.  For simplicity of computation, we set $p=0.5$ here as a lower bound for $P_c$.

\subsubsection{DW Watermark Insertion}
After legalization with placement $P_{lg} = (X_{lg}, Y_{lg})$, cells are moved along the x- or y-axis to insert unique watermark signatures hashed as $N$ bit sequences $B_{N}$, as outlined in Algorithm~\ref{alg:select_cells}. If the $i$-th bit in the signature $B_{N}$ is 1, the cell $c_{i}$ randomly selected from the candidate watermarked cell set $C_x$ is moved along the x-axis for $D_x[c_i]$. If the $i$-th signature bit is 0, the cell $c_{i}$ is randomly chosen from the candidate watermarked cell set $C_y$ and moved along the y-axis for $D_y[c_i]$. 
The resulting placement is denoted as intermediate placement $P_{itr}=(X_{itr}, Y_{itr})$, and the indices of the cells moved along the x- or y-axis form the watermarked cells $C_w$. 
This movement process occurs before detailed placement, allowing possible performance degradation to be compensated during the subsequent detailed placement phase and yield a watermarked solution $P_{wm}=(X_{wm}, Y_{wm})$. 
The selected watermarked cells $C_w$, and their corresponding position distance $\mathrm{Dist} = P_{itr}(C_w)-P_{wm}(C_w)$ between intermediate placement $P_{itr}(C_w)$ and the watermarked placement $P_{wm}(C_w)$ constitute the watermark. 


\noindent\textbf{DW Watermark Strength:} The selection of the watermarked cells from $C_x$  and $C_y$ and the step $|d_x|$ and $|d_y|$ to move is random.
The p-value denoted as $P_c$ to measure the probability of a solution carrying the watermark purely by coincidence can be formulated by Equation~\ref{eq:dp_strength1}. $P_{cx}$ is the probability of cells moving along the x-axis being the same as the watermarked cells, and  $P_{cy}$ is the probability of cells moving along the y-axis being the same as the watermarked cells.  

\begin{equation}
\label{eq:dp_strength1}
\begin{array}{ll}
P_c = P_{cx}  \cdot P_{cy} 
\end{array}
\end{equation}

In Equation~\ref{eq:dp_strength2}, $P_{cx}$ is the probability of $x$ or more cells match the watermarked cells along x-axis as $C_{wx}$, and the $p_x = \frac{|C_{wx}|}{|C_x|}$ is the probability of the watermarked cells $C_{wx}$ are chosen from all of the candidate cells $C_x$. Similarly, $P_{cy}$ is the probability of $y$ or more cells match the watermarked cells along the y-axis, and the $p_y = \frac{|C_{wy}|}{|C_y|}$. Given $|C_x| \gg |C_{wx}|$ and $|C_y| \gg |C_{wy}|$, the above $p_x$ and $p_y$ can be viewed as the approximate probability for no replacement watermarked cell selection. We will give statistical analysis for the designs in Section~\ref{sec:security_ana}. 

\begin{equation}
\label{eq:dp_strength2}
\begin{array}{ll}
P_{cx} = \sum_{i=x}^{|C_{wx}|}\cdot \mathbf{C}(|C_{wx}|, i)  \cdot(p_x)^i \cdot (1-p_x)^{X-i} \\
P_{cy} = \sum_{j=y}^{|C_{wx}|} \cdot \mathbf{C}(|C_{wy}|, j)  \cdot(p_y)^{j} \cdot(1-p_y)^{Y-j}
\end{array}
\end{equation}
%\sum_{i=0}^x C(C_wx, i)\cdot(p_x)^{X-i} \cdot(1-p_x)^i \\ \sum_{j=0}^y  \cdot C(C_y, j) \cdot(p_y)^{Y-i} \cdot(1-p_y)^i

\subsubsection{\textbf{DW Watermark Extraction}}
The design owner detects watermarks in the placement $P^{\prime}$ by comparing the watermarked cell $C_w$ position with the intermediate placement $P_{itr}$ and calculates the new distance $\mathrm{Dist}^{\prime}$ as $P_{itr}(C_w)-P^{\prime}(C_w)$. If $C_w^\prime$ cells in the extracted $\mathrm{Dist}^{\prime}$ matches the $\mathrm{Dist}$ both along x- and y-axis, the watermark extraction rate is calculated as Equation~\ref{eq:dw_wer}.

\begin{equation}
    \label{eq:dw_wer}
   \%WER_{DW} = 100\times\frac{|C_w^\prime|}{|C_{w}|}
\end{equation}
 
\subsection{\sys{} Watermarking} \label{sec:sys}
As a combination of both the GW and the DW, \sys{} applies global watermarking during its global placement stage and detailed watermarking on top of the watermarked region before its detailed placement stage. By combining these two watermarking schemes, the inserted watermark strength is further augmented. 

\begin{figure}[ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/unimarks_wm.pdf}
     \caption{\sys{} framework. \sys{} first applies global watermarking during its global placement and then applies detailed watermarking on top of the watermarked region before the detailed placement.}
    \vspace{-0.5cm}
    \label{fig:unimarks}
\end{figure}
%
\subsubsection{\sys{} Watermark Insertion}
As depicted in Figure~\ref{fig:unimarks}, \sys{} employs a hybrid approach that combines \textit{Global} and \textit{Detailed Watermarking} to produce stronger watermarks. Initially, \sys{} searches the placement for a watermarked region using the strategy akin to \textit{Global Watermarking}, yielding watermarked cells $C_{w1}$ and a watermarked region $K_w$ in the first step. \sys{} runs global placement and legalization with such watermark constraints. Then, it perturbs cells along the x- and y-axis within the watermarked region $K_w$, similar to the approach of \textit{Detailed Watermarking} to obtain an intermediate placement $P_{itr}$. Afterward, the detailed placement proceeds to compensate for watermarking degradation and produce the watermarked placement $P_{wm}$. The perturbed distance $\mathrm{Dist}$ and cells $C_{w2}$ obtained from this process are the watermarks in the second step. 

\noindent\textbf{Watermark Strength:} Due to the combination of global and detailed watermarking, the watermark strength $P_c$ of \sys{} is further augmented. To coincidentally carry the watermark, one has to overcome both the signatures from the global and detailed watermarking. Given the watermark strength of the global watermarking to be $P_{cg}$ and the detailed watermarking to be $P_{cd}$, where the $|C_x|$ and $|C_y|$ are changed to the number of cells available to move in the watermarked region. 
We get the \sys's $P_c$ as in Equation~\ref{eq:sys_strength}, further minimizing the coincidental probability. 

\begin{equation}
    \label{eq:sys_strength}
    P_c=P_{cg}\cdot P_{cd}
\end{equation}

\subsubsection{\sys{} Watermark Extraction}
To claim ownership of the layout, given the cell positions $P^\prime$, the watermark holder can use the following two steps. (i) The extraction of the watermarks $C_{w1}^{\prime}$ from the watermarked region $K_w$, with the global extraction rate denoted as $\%WER_{GW} = 100\times \frac{C_{w1}^{\prime}}{C_{w1}}$. (ii) Afterwards, the inserted signatures are extracted by comparing $P^\prime - P_{itr}$ with $\mathrm{Dist}$ at the watermarked cell indices $C_{w2}$. The number of cells successfully matched is denoted as $C_{w2}^\prime$, from which the detailed extraction rate is calculated as $\%WER_{DW} = 100 \times  \frac{C_{w2}^{\prime}}{C_{w2}}$.   
The final WER is calculated in Equation~\ref{eq:unimark_wer}.

\begin{equation}
\label{eq:unimark_wer}
\begin{array}{ll}
\%WER = 100 \times \frac{WER_{GW} + WER_{DW}}{2}
\end{array}
\end{equation}

%The region extraction rate determines if the placement belongs to the holder, and the cell extraction rate further strengthens the watermark by including unique and confidential signatures.

==> files_backup/5_experiment.tex <==
In this section, we first introduce the experiment setups. Then, we evaluate the watermarking performance of wirelength-driven and timing-driven placement watermarking on different benchmarks and compare it with baselines. Next, we evaluate the robustness of \sys{} under different attacks.  

\subsection{Experiment Setup}

\textbf{Datasets:}
We evaluate the performance of the watermark on three benchmark suites for wirelength-driven placement: ISPD'2005~\cite{nam2005ispd2005}, ISPD'2015~\cite{bustany2015ispd}, and ISPD'2019~\cite{liu2019ispd}; and one benchmark suite for timing-driven placement: ICCAD'2015~\cite{7372671}. All designs in the ICCAD'2015 benchmark suite are large and contain more than 700k cells. It demonstrates the strong applicability of \sys{} in timing-driven placement watermarking. 
The designs with additional fence regions are marked in blue. The statistics of these designs are summarized in Table~\ref{tab:dataset_statistic} in the appendix.

\noindent\textbf{Baseline:} We choose row parity as our baseline~\cite{kahng2001constraint}. It inserts unique bit sequences as watermarks by shifting cells to different rows in the placement stage. Cells with a 1-bit are moved to an odd row, while cells with a 0-bit are moved to an even row. %Routing-based watermarking tends to introduce additional wirelength overhead into the layout, whereas placement-based watermarking can optimize this issue early in the placement stage. Nevertheless, we also include a comparison between routing-based watermarking~\cite{1510323} and \sys{} in the Appendix~\ref{sec:routing_wm_append}.%This approach is designed for partition-based placement, and we re-implement the algorithm on analytical placement algorithms by adding a penalty cost during legalization if the watermarked cell is in the wrong row.

A signature of 50-bit length is used to compare \sys{} against the row parity scheme~\cite{kahng2001constraint}. To successfully prove ownership, the owner not only needs to provide the signatures but also the exact distance information for \sys:DW; cell ID, and region positions for \sys:GW. The watermarking strength, if all watermarks are successfully extracted, is $10^{-15}$ for 
Row Parity, but will be 1.25$\times$$10^{-46}$ for \sys{} because more randomness is added into the signatures as shown in Table~\ref{tab:bits}.  Therefore, this signature provides sufficient protection to the layout. 

\begin{table}[!ht]
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{ccccc}
    \toprule
         & Row Parity~\cite{kahng2001constraint} & GW & DW & \sys \\
        \hline
     10 bits & 1.95$\times$$10^{-3}$ & 1.91$\times$$10^{-6}$ & 9.76$\times$$10^{-24}$ & 1.77$\times$$10^{-15}$  \\
     30 bits & 1.86$\times$$10^{-9}$ & 5.68$\times$$10^{-14}$ & 1.91 $\times$$10^{-55}$ & 4.93$\times$$10^{-32}$ \\
     50 bits & 1.77$\times$$10^{-15}$ & 1.69$\times$$10^{-21}$ & 7.88$\times$$10^{-81}$ & 1.25$\times$$10^{-46}$ \\
     100 bits  & 1.57$\times$$10^{-30}$& 1.50$\times$$10^{-36}$ &  7.88$\times$$10^{-131}$ &  1.43$\times$$10^{-74}$ \\
    \bottomrule
    \end{tabular}
    }
    \caption{Watermarking strength provided by different signature lengths under different watermarking frameworks.}
    \vspace{-0.3cm}
    \label{tab:bits}
\end{table}




%In Section~\ref{subsec:wm_chip}, some related works proposed adding additional routing constraints in the physical design to embed watermarks. However, these techniques are orthogonal to our proposed watermarking scheme. They can be combined to strengthen IP protection.  \textcolor{red}{To Rachel: I think we should think of a better way to show why we are different from the routing things.}

\noindent\textbf{Evaluation Metrics}
For the wirelength-driven placer whose overall quality is measured by the layout wirelength, we use three metrics to evaluate the watermark performance. For \sys, we report $WER = \frac{WER_{GW}+WER_{DW}}{2}$: 

\noindent\textbf{Placement WireLength Rate (PWLR)}: The rate of estimated half-perimeter wirelength (HPWL) of watermarked layout compared to the original layout after placement. 

\noindent\textbf{Routing WireLength Rate (RWLR)}: The rate of routed wirelength of watermarked layout compared to the original layout after routing.

\noindent\textbf{Watermark Extraction Rate (WER)}: The percentage of watermarked cells extracted from the layout. 

%\noindent\textbf{Watermark Overhead (WO)}: The additional time takes to insert watermark compared with non-watermarked layout.

\begin{comment}
Estimated Placement Wirelength Ratio (PWLR) after placement, Routing Wirelength Ratio (RWLR) of the layout, Watermark Extraction Rate (WER), and Watermark Overhead (WO) of the layout. 

\begin{itemize}
    \item Placement Wirelength Ratio (PWLR): The ratio of placement half-perimeter wirelength (HPWL) of watermarked design compared to the original design. %\textcolor{red}{Rachel: HPWL is a common way to estimate placement wirelength and there are other ways to estimate placement wirelength too.}
    \item Routing Wirelength Ratio (RWLR): The ratio of routing wirelength of watermarked design compared to the original design.
    \item Watermark Extraction Rate (WER): The percentage of watermarked cells extracted from the layout. 
    \item Watermark Overhead (WO): The time ratio it takes to perform placement algorithm with watermark insertion compared to non-watermarked placement algorithms.  
%    \item  Watermark Strength ($P_c$): the strength of the watermark. 
\end{itemize}
\end{comment}


For the timing-driven placer, whose overall quality is measured by the timing slack, we add two additional metrics to evaluate the performance using static timing analysis~\cite{huang2020opentimer}: 

\noindent\textbf{Total Negative Slack Rate (TNSR)}: The rate of total negative slack of watermarked layout compared to original one.

\noindent\textbf{Worst Negative Slack Rate (WNSR)}:The rate of worst negative slack of watermarked layout compared to original one.

%\noindent\textbf{Wirelength Ratio (WLR):} The ratio of placement wirelength of watermarked design compared to the original design. 
%\textcolor{blue}{change to geo-mean}
%We report their \textbf{G-Avg} by multiplying the weighted number of cells with the metrics to obtain their average.
To preserve the optimized outcomes from the physical design algorithms, we set a threshold of layout quality degradation to not exceed 0.5\%. Because surpassing this threshold would counteract the benefits derived from the performance enhancement efforts in physical design.

\begin{comment}
\begin{itemize}
    \item Total Negative Slack Ratio (TNSR): The ratio of timing-driven total negative slack of watermarked design compared to the original design.
    \item Worst Negative Slack Ratio (WNSR): The ratio of timing-driven worst negative slack of watermarked design compared to the original design.
    \item Placement Wirelength Ratio (PWLR): The ratio of placement half-perimeter wirelength (HPWL) of watermarked design compared to the original design. %\textcolor{red}{Rachel: HPWL is a common way to estimate placement wirelength and there are other ways to estimate placement wirelength too.}
    \item Watermark Extraction Rate (WER): The percentage of watermarked cells extracted from the layout. 
  %  \item Watermark Overhead (WO): The time ratio it takes to perform placement algorithm with watermark insertion compared to non-watermarked placement algorithms.  
%    \item  Watermark Strength ($P_c$): the strength of the watermark. 
\end{itemize}
\end{comment}

\subsection{Results}


\subsubsection{Wirelength-driven Placement Watermarking}



\input{files/table/all_tab}
The performance of different watermarking schemes is tabulated in Table~\ref{tab:ispd2005} for the ISPD'2005 benchmarks~\cite{nam2005ispd2005}, in Table~\ref{tab:ispd2015} for the ISPD'2015 benchmarks~\cite{bustany2015ispd}, and in Table~\ref{tab:ispd2019} for the ISPD'2019 benchmarks~\cite{liu2019ispd}. 
For all the layouts in Table~\ref{tab:ispd2005}-Table~\ref{tab:ispd2019}, their inserted watermarks can be successfully extracted. Therefore, we evaluate how much layout performance degradation is compromised to accommodate such watermark insertion among these watermarking algorithms.

%\textbf{Our research question is: to have these watermarks successfully embedded, how much quality of the designs should be compromised to accommodate those watermarks?}
 
From the tables, we can make the following observations: 

\noindent\textbf{Comparison with Row Parity}~\cite{kahng2001constraint}: Across all three benchmark suites, both \sys{} and its two submodules, \sys: GW and \sys: DW, exhibit reduced performance degradation compared to Row Parity. When assessing the placement Half-Perimeter WireLength Rate (PWLR), there is a relative reduction by 0.54\%, 0.39\%, and 0.76\% for \sys: GW, \sys: DW, and \sys{}, respectively, against Row Parity across the benchmarks. Similarly, the average routed wirelength rate (RWLR) demonstrates a reduction of 2.60\%, 2.12\%, and 2.63\% for \sys: GW, \sys: DW, and \sys{}, respectively. Notably, the gap in wirelength degradation between \sys{} (including its submodules) and Row Parity becomes more pronounced after routing. This is attributed to the fact that Row Parity relocates cells to different rows, necessitating the router to traverse multiple rows to connect to the watermarked cell.

%It means after routing, the actual wirelength improvement compared with non-watermarked designs improved by 4 $\times$ to 7 $\times$ for the Row Parity watermarking, whereas 

%the Row Parity watermarking is becoming 4 $\times$ to 7 $\times$ larger compared with the estimation from placement outputs. 

\noindent\textbf{Comparison with GW and DW:} As a combination of GW and DW, \sys{} takes advantage of their strength and further reduces the performance degradations from accommodating watermarks. The average PWLRs on ISPD'2005, ISPD'2015, and ISPD'2019 are reduced by 0.22\% and 0.37\% compared with the \sys: GW and \sys: DW. The average RWLRs on ISPD'2015 and ISPD'2019 are reduced by 0.03\% and 0.51\% compared with \sys: GW and \sys: DW, respectively.

Compared with DW, \sys{} improves the solution because DW chooses cells to move across the layout. Some watermarked cells in DW are in compact areas, and moving them results in huge performance degradation. For \sys, the cells to move are in less compact regions identified by GW, making \sys's watermark insertion yield less performance degradation. 

In contrast to GW, \sys{} improves the placement quality. This improvement stems from modifying cell positions within a designated region, either across different rows or along the x-axis. Such modifications inherently disturb solutions formulated during global placement. Given that these disturbances occur in less compact regions, they provide different inputs to the detailed placement process, thereby offering potential optimization trajectories to minimize overall wirelength. It's pivotal to note that while the detailed watermarking suggests possible optimization avenues, the magnitude of improvement to GW depends on the quality of the perturbations introduced.
As can be seen from the tables, the improvement on ISPD'2019 is slight, with 0.03\% reduction in PWLR and 0\% reduction in RWLR. However, the improvements in the ISPD'2005 and ISPD'2015 are much larger. The PWLR is reduced by 0.23\% and 0.39\% for ISPD'2005 and ISPD'2015, and RLWR is reduced by 0.05\% for ISPD'2015.

\noindent\textbf{Performance with additional design constraint:} For layouts with fence region as additional constraints, accommodating the watermarks becomes more challenging. As shown in Table~\ref{tab:ispd2015}, the PWLR of designs with fence region is increased by 0.01\% - 0.78\%, and the RWLR of designs with fence region is increased by 0.06\% - 1.14\% for all watermarking methods. 

After routing, the RWLR of Row Parity is 1.0327 and significantly over the 0.5\% threshold, compromising the additional effort the design company invests to optimize the physical design algorithms. For \sys{} and its two submodules, however, the RWLR improvement over the non-watermarked layouts are 0.29\%, 0.12\%, and 0.01\%, which still maintains good layout quality after watermark insertion. 

% 1.0024-1.002 + 1.0043-0.9946 + 1.0065-1.0003
% 1.0024-1.0006 + 1.0043-1.0007 + 1.0065-1.0001
% 1.0024-0.9997 + 1.0043-0.9909 + 1.0065-0.9996
% 1.0234-0.9914+1.0196-0.9996
% 1.0234-1.0006+1.0196-1.0001
% 1.0234-0.9909+1.0196-0.9996

%\textcolor{red}{To Rachel: I changed the WO to $T_{wm}$ - $T_{ori}$ and report the extra time takes to wm. I think it's more convincing, how do you think?}

%Given the average of XX\% PWLR and XX\% RWLR improvement over the non-watermarked design, XX\% watermarking overhead is acceptable. Besides, with the GPU accelerated placement library provided by DREAMPlace~\cite{lin2019dreamplace}, the maximum time takes to place the design is less than XX minutes, meaning the additional time overhead to insert watermark is less than XX minutes. 
%\textcolor{red}{To Rachel: Do you think current watermark overhead looks decent for GW \& Unimarks? Split the run-time into two part: (i) finding cells; (ii) add total runtime; (iii) change WO to 2 decimal (iv) highlight WO} 



\input{files/table/iccad2015}
\subsubsection{Timing-driven Placement Watermarking}

To evaluate the impact of placement watermarking on a layout's timing metric, we employ a timing-driven placer, DREAMPlace 4.0~\cite{9774725}.
A timing-driven placement algorithm targets to meet the specified timing constraint for the layout by moving cells on timing-critical paths closer to each other.
Meeting the timing constraint is prioritized over minimizing the overall wirelength of the layout.

Experiments on the ICCAD'2015 \textit{superblue} designs are reported in Table~\ref{tab:iccad2015}. From the table, we find that \sys{} achieves the lowest performance degradation on all watermarking targets. Compared with the baseline Row Parity~\cite{kahng2001constraint}, the average TNSR is reduced by 7.48\%, WNSR is reduced by 2.84\%, and PWLR is reduced by 0.35\%. \sys{} also achieves 0.82\% TNSR improvement compared with the best-performing results on its two submodules DW and GW. It proves that \sys{} can maintain the layout quality when more optimization objectives, i.e., timing metrics, are included in the physical design.  For more results regarding its performance under attacks, please refer to the additional experiments section in Appendix~\ref{sec:attack_timing_append}.



\subsubsection{Watermarking Capacity}


In this subsection, we explore the maximum length of watermark bits, i.e. watermarked cells, that can be inserted into the layout without degrading the quality. We use the ISPD'2019 benchmark~\cite{liu2019ispd} as an example and show the maximum bits that can be embedded. For detailed watermarking and row parity, the signature length corresponds to the moved cell number to satisfy the watermark insertion constraints. For global watermarking, the signature length corresponds to the $|N_w|$. It is the total number of cells in the watermarked region as defined in Equation~\ref{eq:score}. For \sys, the signature length corresponds to the $|N_w|$ cells in global watermarking and moves $|N_w|$ cell in the watermarked region to insert signatures in the detailed watermarking. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width= \columnwidth]{figs/capacity.pdf}
     \caption{Watermarking capacity for different frameworks on ISPD'2019 benchmarks~\cite{liu2019ispd}. We consider the threshold for acceptable degradation of layout quality as 0.5\%.}%\textcolor{red}{extend to 100k and 200k. like 5\% of the cells(see what's happen for specific layout.change different marker for two sets.=)}
    %\vspace{-0.5cm}
    \label{fig:capacity}
\end{figure}

As shown in Figure~\ref{fig:capacity}, we evaluate the signatures with lengths set to 30 bits, 50 bits, 100 bits, 200 bits, 500 bits, and 1000 bits. As the signature becomes larger, accommodating more bit sequences into the layout becomes harder for row parity and detailed watermarking. This is because more cells are moved across the layout and degrade layout quality. However, for global watermarking and \sys, exploring the less compact region and inserting signatures within the region minimizes performance degradation. Therefore, it helps to accommodate watermarks with larger signature lengths. 

Since \sys{} builds the watermarking scheme on top of global watermarking, the two PWLR and RWLR lines overlap in Figure~\ref{fig:capacity}. 
For Row Parity, the RWLR is much higher than its PWLR because when cells are moved to a different row, the router has to cross rows to connect the watermarked cell. Therefore, the actual routed wirelength is much higher. The maximum bits that can be inserted by Row Parity and \sys:DW are 30 bits and 100 bits, respectively. However, for \sys:GW and \sys, the maximum number of signatures that can be inserted goes up to over 200 bits. 
 



\subsection{Security Analysis}\label{sec:security_ana} 

\subsubsection{Attack Evaluations}
We analyze the resilience of watermarking schemes, including row parity~\cite{kahng2001constraint}, \textit{Global Watermarking} (GW), \textit{Detailed Watermarking} (DW), and \sys{} toward three aforementioned attacks: ghost attack, removal attack, and denial attack as listed in Table~\ref{tab:security}. The \xmark{} denotes that the watermarking scheme is not resilient to the attack, and \cmark{} means resilience. 




\begin{table}[!ht]
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{ccccc}
    \toprule
         & Row Parity~\cite{kahng2001constraint} & GW & DW & \sys \\
        \hline
      Ghost Attack  & \xmark & \cmark & \cmark  & \cmark\\
      Denial Attack & \cmark  & \cmark & \cmark & \cmark\\
     Average $P_c$ & 1.77$\times$$10^{-15}$ & 1.69$\times$$10^{-21}$ & 7.88$\times$$10^{-81}$ & 1.25$\times$$10^{-46}$ \\
      Removal Attack   & \cmark & \cmark& \cmark & \cmark\\
    \bottomrule
    \end{tabular}
    }
    \caption{Security Analysis of Watermarking Schemes. The watermarking signature length for calculating $P_c$ is 50 bits.}

    \label{tab:security}
\end{table}
\paragraph{Ghost Attack:} In ghost attacks, the adversary 
extracted another set of watermarks from the design company's layout as ghost watermark. The adversary claims his ownership of the layout by asserting the inserted watermark in the layout is the ghost watermark. 
The row parity watermarking method in Table~\ref{tab:security} is not resilient to ghost attacks. If an adversary understands how the placement is watermarked without knowing the exact signature, they can easily counterfeit a different set of ghost watermark signatures from the row index ID of cells and claim the watermark belongs to them. 

%This challenges the design company, who lacks mechanisms to authenticate whether they have genuinely watermarked the cell indexes. 

\textit{Global Watermarking} exhibits resilience to ghost attacks because the region with the minimal evaluation score is unique in the original placement, and the scoring parameters are kept confidential. It is hard for adversaries to fake or find another set of ghost watermarks with only access to the watermarked layout. Even if the adversary has access to the watermarking coefficients and the watermarked layout, the searched region differs from performing the same scoring mechanism on the original layout (See ARA attack in Section~\ref{sec:removal_attack} for more details). 
As the watermarks are inserted during global placement, to counterfeit the watermark, the adversaries can only re-run the placement and routing stages to add his own signatures. However, running those stages without access to the optimized constraints found by the design company could greatly degrade the layout performance. 

\textit{Detailed Watermarking} is resistant to ghost attacks because asserting ownership requires the watermarked cells and the distance $\mathrm{Dist}$ between the watermarked placement and the intermediate placement. The intermediate placement is obtained after legalization, making it exceedingly difficult to counterfeit $P_{itr}$. \sys{}, as a combination of DW and GW is also resilient to ghost attacks. 


\paragraph{Denial Attack:} In the denial attack, the adversary claims the watermark is a coincidental by-product of the physical design. The possibility of the coincidental layout can be measured by the watermark strength $P_c$. The lower the $P_c$ is, the less possibility the layouts are subject to denial attacked. We calculate the $P_c$ of \sys{} and its two submodules based on Equation~\ref{eq:gp_strength}-\ref{eq:sys_strength}.We calculate the probability that a layout has the same watermark signature by coincident and report the average $P_c$ on three benchmarks in the third row of Table~\ref{tab:security}, where all possibilities are close to 0. It means the watermarks in the layouts are not coincidental and cannot be denied. 


\paragraph{Removal Attack:} In the removal attack, the adversary attacks the layout by removing the watermarks.  
The row parity watermarking method is resilient to removal attacks. Since the number of cells scales into the millions in modern designs, discerning which cells are watermarked and moving them to another row to eliminate the signature is nearly impossible. For \textit{Detailed Watermarking}, to remove the signature, an adversary would have to perturb a large fraction of cells, significantly degrading placement performance. %The significant quality degradation will compromise the additional effort spent by the design company to optimize the physical design algorithms. 
This also applies to \textit{Global Watermarking}, where the adversaries would have to relocate all the $C_w$ cells out of the watermarked region, which significantly degrades the placement quality. \sys{}, as a combination of DW and GW, is also resilient to removal attacks. We also systematically analyze their resiliency to different removal attacks in Section~\ref{sec:removal_attack}. 
 
%This scheme is also resilient to removal attacks as adversaries would have to relocate all the $C_w$ cells out of the watermarked region, which significantly degrades the placement quality. For denial attacks, we can find the watermark strength $P_c$ is close to 0, meaning the design is almost impossible to be denial attacked. 

%\textit{Detailed Watermarking} in Table~\ref{tab:security} is resistant to both denial and ghost attacks because asserting ownership requires not only the watermarked cells but also the distance $\mathrm{Dist}$ between the watermarked placement and the intermediate placement. The intermediate placement is obtained after legalization, making it exceedingly difficult to counterfeit $P_{itr}$. Furthermore, to remove the signature, an adversary would have to perturb a large fraction of cells, leading to a significant degradation in placement performance, rendering the placement unsuitable for later manufacturing.

%\sys{}, as a combination of \textit{Detailed Watermarking} and \textit{Global Watermarking} in Table~\ref{tab:security}, inherits the advantages of both schemes and thus is resilient to all three types of attacks.


\subsubsection{Removal Attack Evaluation}\label{sec:removal_attack}

In this subsection, we evaluate the resilience of watermarking algorithms against removal attacks and quantitatively demonstrate the results. While these attacks seek to remove watermarks, the layout must remain in good quality post-attack.
As any degradation of placement Half-Perimeter WireLength Rate (PWLR) and routed wirelength rate (RWLR) directly results in increased area and manufacturing costs, we restrict any PWLR and RWLR increase, compared to the non-watermarked placement, to $<0.5\%$. We set a PWLR and RWLR threshold as 1.005, represented by the black dotted line in the left two subfigures of Figure~\ref{fig:attack_results}. To successfully claim ownership of the layout, we set the watermark extraction rate (WER) threshold to 90\%, represented as the black dotted line in the rightmost subfigure of Figure~\ref{fig:attack_results}.



We benchmark the resilience of different watermarking frameworks on ISPD'2005~\cite{nam2005ispd2005}, ISPD'2015~\cite{bustany2015ispd}, and ISPD'2019~\cite{liu2019ispd} benchmarks to compare resilience under four types of removal attacks aiming to prevent the placement owner from proofing ownership: (i) swap location attacks (SLA) by ~\cite{kahng2001constraint} which target to attack Row Parity framework, (ii) constraint perturbation attacks (CPA) which target to attack DW and \sys{} framework; (iii) Optimization attacks (OA) which target to attack all watermarking frameworks; and (iv) adaptive region attacks (ARA) which target to attack GW and \sys{} framework. %While these attacks are designed to attack specifically some of the algorithms, we show the performance of all of the watermarking frameworks. 
The results are summarized in Figure~\ref{fig:attack_results}. Additional attacks on layout generated by the timing-driven placers are included in the appendix Section~\ref{sec:attack_timing_append}.

%https://colab.research.google.com/drive/1dE2ISh1IGwYpOYN_Bg7rfXlTMKRqmVwu?usp=sharing


\begin{figure*}[!ht]
    \centering
    \subfloat[Swap location attack (0.1\% cells) ]{\label{f:sla_10_attack} \includegraphics[width=0.5\linewidth]{figs/SLA_10.pdf}}
    \subfloat[Swap location attack (0.5\% cells) ]{\label{f:sla_50_attack} \includegraphics[width=0.5\linewidth]{figs/SLA_50.pdf}} \\
    \subfloat[Constraint perturbation attack (0.1\% cells) ]{\label{f:cpa_0.001} \includegraphics[width=0.5\linewidth]{figs/CPA_0.001.pdf}} 
    \subfloat[Constraint perturbation attack (1\% cells) ]{\label{f:cpa_0.01} \includegraphics[width=0.5\linewidth]{figs/CPA_0.01.pdf}} \\
    \subfloat[Constraint perturbation attack (10\% cells)]{\label{f:cpa_0.1} \includegraphics[width=0.5\linewidth]{figs/CPA_0.1.pdf}} 
    \subfloat[Optimization attack ]{\label{f:eco_attack} 
    \includegraphics[width=0.5\linewidth]{figs/ECOA.pdf}} \\
    \subfloat[Adaptive region attack (top-1) ]{\label{f:ada_attack1} \includegraphics[width=0.5\linewidth]{figs/ARA.0.1.pdf}}
   \subfloat[Adaptive region attack (top-5) ]{\label{f:ada_attack5} \includegraphics[width=0.5\linewidth]{figs/ARA.0.5.pdf}}
    \caption{Watermarking performance of different frameworks under attacks. The black dotted line in the two left subfigures denotes the quality degradation threshold as 1.005, and the black dotted line in the rightmost subfigure denotes the watermark extraction threshold as 90\%. In the legend, WL is short for wirelength, and WE is short for watermark extraction.}
  
    \label{fig:attack_results}
\end{figure*}

%\ruisi{Say Percentage instead of 10 cells, run with detail placement. given an average of how many cells are moved in SLA and CPA; Have different color for WER, have common legend; Add another attack, attacker knows we have done a region, he tries to mess up top-3/5. } \textcolor{red}{To Rachel: Could you check if the WER and dotted line look descent this time? (i) Add a scenario where Row Parity is really bad.}

\paragraph{Swap Location Attacks (SLA):}
In SLA~\cite{kahng2001constraint}, cells randomly exchange their locations with another set of cells. Then, a follow-up legalization and external detailed placement engine compensate for the performance degradation and ensure the cells follow the design rules. 
In Figure~\ref{f:sla_10_attack} and Figure~\ref{f:sla_50_attack}, we randomly choose 0.1\% and 0.5\% cells from the layout and pair them to exchange their locations. From here, we can find even small location swaps result in huge performance degradation on modern IC layouts.  In terms of the watermark extraction, Row Parity, and \sys:DW get WER below 90\% and failed to verify their ownership. This is because \sys:DW and Row Parity's watermarks spread the placement, and some of the watermarked cells can reside in the compact area. Minor changes will subsequentially modify most cell locations within the compact region. Therefore, the watermarks represented as cell locations are altered for both approaches. 
By embedding cells in the less compact region, \sys:GW and \sys{} are less sensitive to such changes.  
Therefore, \sys:GW and \sys{} still maintain high WER. 


\paragraph{Constraint Perturbation Attacks (CPA):}
In CPA, cells shift their location along the x- or y-axis if space is available. In Figure~\ref{f:cpa_0.001}, Figure~\ref{f:cpa_0.01}, and Figure~\ref{f:cpa_0.1}, we move the positions of 0.1\%, 1\%, 10\% of the cells have ample space to move in the layout. 
From here, we find that under CPA 0.1\% attack, layout performance hit the boundary of the performance degradation threshold. In ISPD'2015 and ISPD'2019, the placement wirelength and routed wirelength degradations are close to 0.5\%. For the watermark extraction, both the \textit{Global Watermarking} and \sys{} achieve over 90\% WER. For the CPA 1\% and 10\% cell performance, however, the PWLR and RWLR degradations are greater than 5\%, meaning the attack failed to maintain the layout quality improvement from the design company's physical design optimizations. But \textit{Global Watermarking} and \sys{} still maintain higher than 90\% WER and successfully help the design company to claim ownership of the layout. 
 
\paragraph{Optimization Attacks (OA):}
This attack employs an additional optimization stage to remove the watermarks.
The optimization is implemented through another round of detailed placement from an open-source placer to remove the watermark. Here, we use NTUPlace3~\cite{4544855} as an external detailed placement engine to attack the ISPD'2005 benchmark and NTUPlace4dr~\cite{7940087} as an external detailed placement engine to attack the ISPD'2015 and ISPD'2019 benchmarks. It aims to change cell locations slightly to remove watermarks while maintaining the layout quality.  From Figure~\ref{f:eco_attack}, we can find that the layout quality degradations in all three benchmarks remain below 1.005. For the watermark extraction, all of the watermarking frameworks achieve over 90\% WER. It indicates OA failed to attack the layouts. 

\paragraph{Adaptive Region Attacks (ARA):}
This attack assumes the adversary's target is the \sys's watermarking framework. He has prior knowledge of how \sys{} performs the watermarking and has access to the coefficients used to search the watermarked region. The adversary operates on top of the watermarked layout. He 
tries to remove the inserted watermarks by moving cells within the searched top-1 or top-5 regions if there is room.

In Figure~\ref{f:ada_attack1} and Figure~\ref{f:ada_attack5}, we can find that the PWLR and RWLR degradations are minimal and below the 0.5\% threshold for most of the watermarking frameworks.  For the watermark extraction, \sys:GW and  \sys{} methods achieve over 90\% WER, whereas Row Parity and \sys:DW failed to provide ownership proof in the ARA Top-5 settings. This is because \sys:GW and \sys{}' watermarks are encoded as a co-optimization term in the global placement stage; the top regions found by the scoring function on the watermarked layout are not the same one as the watermarked region.  However, the watermarks of Row Parity and \sys:DW are spread among the layout, where minor changes in the compact area will subsequentially modify the inserted watermarks. Therefore, the two frameworks' WER are compromised.


%\racheltodo{We claim 100\% extraction in the contributions, but here it is > 90\%. Is this enough?}




\noindent\textbf{Comparison with Row Parity}~\cite{kahng2001constraint}: Across all three benchmark suites, both \sys{} and its two submodules, \sys: GW and \sys: DW, exhibit reduced performance degradation compared to Row Parity. When assessing the placement Half-Perimeter WireLength Rate (PWLR), there is a relative reduction by 0.54\%, 0.39\%, and 0.76\% for \sys: GW, \sys: DW, and \sys{}, respectively, against Row Parity across the benchma3rks. Similarly, the average routed wirelength rate (RWLR) demonstrates a reduction of 2.60\%, 2.12\%, and 2.63\% for \sys: GW, \sys: DW, and \sys{}, respectively. Notably, the gap in wirelength degradation between \sys{} (including its submodules) and Row Parity becomes more pronounced after routing. This is attributed to the fact that Row Parity relocates cells to different rows, necessitating the router to traverse multiple rows to connect to the watermarked cell.

%It means after routing, the actual wirelength improvement compared with non-watermarked designs improved by 4 $\times$ to 7 $\times$ for the Row Parity watermarking, whereas 

%the Row Parity watermarking is becoming 4 $\times$ to 7 $\times$ larger compared with the estimation from placement outputs. 

\noindent\textbf{Comparison with GW and DW:} As a combination of GW and DW, \sys{} takes advantage of their strength and further reduces the performance degradations from accommodating watermarks. The average PWLRs on ISPD'2005, ISPD'2015, and ISPD'2019 are reduced by 0.22\% and 0.37\% compared with the \sys: GW and \sys: DW. The average RWLRs on ISPD'2015 and ISPD'2019 are reduced by 0.03\% and 0.51\% compared with \sys: GW and \sys: DW, respectively.

Compared with DW, \sys{} improves the solution because DW chooses cells to move across the layout. Some watermarked cells in DW are in compact areas, and moving them results in huge performance degradation. For \sys, the cells to move are in less compact regions identified by GW, making \sys's watermark insertion yield less performance degradation. 

In contrast to GW, \sys{} improves the placement quality. This improvement stems from modifying cell positions within a designated region, either across different rows or along the x-axis. Such modifications inherently disturb solutions formulated during global placement. Given that these disturbances occur in less compact regions, they provide different inputs to the detailed placement process, thereby offering potential optimization trajectories to minimize overall wirelength. It's pivotal to note that while the detailed watermarking suggests possible optimization avenues, the magnitude of improvement to GW depends on the quality of the perturbations introduced.
As can be seen from the tables, the improvement on ISPD'2019 is slight, with 0.03\% reduction in PWLR and 0\% reduction in RWLR. However, the improvements in the ISPD'2005 and ISPD'2015 are much larger. The PWLR is reduced by 0.23\% and 0.39\% for ISPD'2005 and ISPD'2015, and RLWR is reduced by 0.05\% for ISPD'2015.

\noindent\textbf{Performance with additional design constraint:} For layouts with fence region as additional constraints, accommodating the watermarks becomes more challenging. As shown in Table~\ref{tab:ispd2015}, the PWLR of designs with fence region is increased by 0.01\% - 0.78\%, and the RWLR of designs with fence region is increased by 0.06\% - 1.14\% for all watermarking methods. 

After routing, the RWLR of Row Parity is 1.0327 and significantly over the 0.5\% threshold, compromising the additional effort the design company invests to optimize the physical design algorithms. For \sys{} and its two submodules, however, the RWLR improvement over the non-watermarked layouts are 0.29\%, 0.12\%, and 0.01\%, which still maintains good layout quality after watermark insertion. 

% 1.0024-1.002 + 1.0043-0.9946 + 1.0065-1.0003
% 1.0024-1.0006 + 1.0043-1.0007 + 1.0065-1.0001
% 1.0024-0.9997 + 1.0043-0.9909 + 1.0065-0.9996
% 1.0234-0.9914+1.0196-0.9996
% 1.0234-1.0006+1.0196-1.0001
% 1.0234-0.9909+1.0196-0.9996

%\textcolor{red}{To Rachel: I changed the WO to $T_{wm}$ - $T_{ori}$ and report the extra time takes to wm. I think it's more convincing, how do you think?}

%Given the average of XX\% PWLR and XX\% RWLR improvement over the non-watermarked design, XX\% watermarking overhead is acceptable. Besides, with the GPU accelerated placement library provided by DREAMPlace~\cite{lin2019dreamplace}, the maximum time takes to place the design is less than XX minutes, meaning the additional time overhead to insert watermark is less than XX minutes. 
%\textcolor{red}{To Rachel: Do you think current watermark overhead looks decent for GW \& Unimarks? Split the run-time into two part: (i) finding cells; (ii) add total runtime; (iii) change WO to 2 decimal (iv) highlight WO} 



\input{./table/iccad2015}
\subsubsection{Timing-driven Placement Watermarking}

To evaluate the impact of placement watermarking on a layout's timing metric, we employ a timing-driven placer, DREAMPlace 4.0~\cite{9774725}.
A timing-driven placement algorithm targets to meet the specified timing constraint for the layout by moving cells on timing-critical paths closer to each other.
Meeting the timing constraint is prioritized over minimizing the overall wirelength of the layout.

Experiments on the ICCAD'2015 \textit{superblue} designs are reported in Table~\ref{tab:iccad2015}. From the table, we find that \sys{} achieves the lowest performance degradation on all watermarking targets. Compared with the baseline Row Parity~\cite{kahng2001constraint}, the average TNSR is reduced by 7.48\%, WNSR is reduced by 2.84\%, and PWLR is reduced by 0.35\%. \sys{} also achieves 0.82\% TNSR improvement compared with the best-performing results on its two submodules DW and GW. It proves that \sys{} can maintain the layout quality when more optimization objectives, i.e., timing metrics, are included in the physical design.  For more results regarding its performance under attacks, please refer to the additional experiments section in Appendix~\ref{sec:attack_timing_append}.

==> files_backup/5_experiment_backup.tex <==
%%%%%%%%%%%%
%The detailed statistics are summarized in Table~\ref{tab:ispd2005}-Table~\ref{tab:ispd2019}. For the first nine designs in ISPD'2015 and \texttt{ispd19test5} in ISPD'2019, there are extra fence regions as additional optimization constraints. For other designs, there is no such constraints. 


\subsection{Experiment Setup and Parameter Settings}
\sys{} is implemented with Python 3.9 and benchmarked on a Linux Ubuntu system equipped with four NVIDIA TITAN Xp GPUs, each with 12 GB RAM, and 48 Intel(R) Xeon(R) CPUs, accompanied by 128 GB RAM.
Although the watermarking methodology of \sys{} can be integrated into any VLSI placement framework, we chose to build upon the open-source placement framework, DREAMPlace~\cite{lin2019dreamplace}, to demonstrate its viability.
 
By default, in \textit{Global Watermarking}, our sliding window's size is set to 10-row heights both in width and height, and the sliding window stride is set to 5-row heights. The size and stride change with different designs and  are summarized in Table~\ref{tab:ispd2005}-\ref{tab:ispd2019}.
As for the scoring parameters, we set the default values of $\alpha$ = 0.1, $\beta$ = 0.1, and $\gamma$ = 1. In the \textit{Detailed Watermarking} phase, $d_x$ is set to one unit, and $d_y$ is set to 1-row height.


\subsection{Datasets and Baselines}
r In these designs, placement fence regions are indicated in blue in Tables~\ref{tab:ispd2005} to \ref{tab:ispd2019}.

The row parity watermark algorithm~\cite{kahng2001constraint} is considered as the baseline.
It inserts unique bit sequences as watermarks by shifting cells to different rows. Specifically, cells with a 1-bit are moved to an odd row, while cells with a 0-bit are moved to an even row. This approach is designed for partition-based placement, and we re-implement the algorithm on analytical placement algorithms by adding a penalty cost during legalization if the watermark cell is in the wrong row.


\subsection{Evaluation Metrics}

We use two metrics to evaluate the watermark performance: HPWL ratio (WLR) and watermark extraction rate (WER). For \sys, we report $WER = \frac{WER_{region}+WER_{cell}}{2}$. 
\begin{itemize}
    \item HPWL Ratio (WLR): The ratio of HPWL of watermarked design compared to the original placement.
    \item WM Extraction Rate (WER): The percentage of watermarked cells successfully extracted. 
\end{itemize}

\subsection{Benchmarking Results}
 
The performance of the various watermarking schemes is tabulated in Table~\ref{tab:ispd2005} for the ISPD'2005 benchmarks~\cite{nam2005ispd2005}, in Table~\ref{tab:ispd2015} for the ISPD'2015 benchmarks~\cite{bustany2015ispd}, and in Table~\ref{tab:ispd2019} for the ISPD'2019 benchmarks~\cite{liu2019ispd}.

A signature of 50-bit length is used to compare the proposed watermarking schemes against the row parity scheme~\cite{kahng2001constraint} in terms of WLR and WER.
 
From the tables, we can make the following observations: 
\todo{1. add routing metric wl, compare with the row parity to see the final performance}

\begin{itemize}
    \item For all watermarking schemes, the WER is 100\%, meaning all of the watermarks are successfully extracted. 

    \item   Compared to GW, \sys{} consistently achieves better HPWL across all benchmarks. GW degrades placement performance in ISPD'2005 and ISPD'2019 benchmarks, whereas \sys{} maintains the high-quality results. This is attributed to the second step of \textit{Detailed Watermarking} in \sys{}, which effectively compensates for the overall quality degradation caused by GW.

    \item  In comparison to DW and row parity, \sys{} demonstrates higher placement quality across all benchmarks. While row parity and DW introduce watermarking during legalization and before detailed placement, which significantly reduces performance degradation, \sys{} further enhances the process by identifying regions that contribute less to the overall placement's degradation. As a result, \sys{} maintains the overall placement quality without compromising it.
    \item   For benchmarks where fence regions are included as additional optimization objectives in Table~\ref{tab:ispd2015}, we find the row parity watermarking yields worse WLR, and some of the designs have WLR degradation of $> 0.5\%$ compared with the original placement, such as \texttt{des\_perf\_b} and \texttt{pci\_bridge32\_a}. \sys{}, however, still maintains high quality with an average WLR of 0.9972. 
    \item  As the number of cells in the design scales up, \sys{} still achieves better placement quality than the baseline row parity~\cite{kahng2001constraint}. For instance, for \texttt{superblue12} in ISPD'2015, \texttt{ispd19test9} and \texttt{ispd19test10} in ISPD'2019 consisting of millions of cells, the WLR of \sys{} is better than that of row parity. We note that there are cases like \texttt{bigblue3} and \texttt{bigblue4} in the ISPD'2005 benchmark where the WLR of \sys{} is higher than row parity. Upon investigation, we found that the reduced quality primarily stems from a large number of macros spreading the placement. Their dense connections cause the degradation to increase. However, as an alternate solution, we found that detailed placement watermarking still has a high extractability and results in only 0.01\% performance degradation, whereas row parity degrades performance by an average of 0.25\% compared with the non-watermarked placements.
\end{itemize}


\input{files/table/all_tab}

\subsection{Attack Evaluation}

\textcolor{blue}{1. move designs statistics as a separate tables1; move parameters as a seperate table2; 2. Take the average of all design results as y-axis. 3. Change animate ECO using NTUplace placer attack}

While the potential for denial and ghost attacks has been discussed in Section~\ref{sec:security_ana}, in this subsection, we evaluate the resilience of watermarking algorithms against removal attacks and quantitatively demonstrate the results. Although these attacks seek to remove watermarks, the placement must remain usable post-attack.
As any degradation of HPWL directly results in increased area and manufacturing costs, we restrict any HPWL increase, compared to the original placement, to $<0.5\%$.
Thus we set a WLR threshold as 1.005, represented by the black dotted line in Figure~\ref{fig:attack}.



\begin{figure*}[ht]
  \begin{center}
{\label{fig:attack_ada1_hpwl}\includegraphics[width=\linewidth]{figs/degrade.pdf}}
    \\
    {\label{fig:de}\includegraphics[width= \linewidth]{figs/extract.pdf}}
  \end{center}
 
  \caption{
 Watermarkings' resilience against swap location attack (SLA) and constraint perturbation attack (CPA).  $\text{SLA}_{10}$, and $\text{SLA}_{50}$: 10 and 50 cells are selected for SLA;  $\text{CPA}_{0.1\%}$, $\text{CPA}_{1\%}$, and $\text{CPA}_{10\%}$: 0.1\%, 1\%, and 10\% cells are selected for CPA.
  }\vspace{-0.2cm}
  \label{fig:attack}
\end{figure*}


We select three designs: \texttt{mgc\_fft\_a} (34K cells) and \texttt{superblue12} (1293K cells) in ISPD'2015~\cite{bustany2015ispd}, and \texttt{adaptec1} (211K cells) in ISPD'2005~\cite{nam2005ispd2005}, to compare resilience under four types of removal attacks aiming to prevent the placement owner from proofing ownership: (i) swap location attacks (SLA) by ~\cite{kahng2001constraint} (ii) constraint perturbation attacks (CPA); (iii) detailed optimization attacks (DOA); and (iv) adaptive attacks (AA). 

We display the WLR and WER of different watermarking schemes against attacks in Figure~\ref{fig:attack}. We note that when removal attacks significantly degrade the placement quality, both the \sys{} and GW performance tend to converge to similar points, as illustrated in WLR in Figure~\ref{fig:attack}. This convergence occurs because \sys{} primarily perturbs a small fraction of cells upon GW placements, whereas substantial degradation leads to changes in the position of a larger fraction of cells.

\subsubsection{Swap Location Attacks (SLA)}

In this attack, cells randomly exchange their location with another set of cells.
We find that: (i) \textit{Global Watermarking} (GW) demonstrates resilience to various attacks, maintaining a 100\% WER under all attack scenarios. \sys{} inherits this advantage for region extraction, successfully retrieving all the cells within the watermark region. (ii) \textit{Detailed Watermarking} (DW), however, exhibits a trade-off between quality and extraction rates.  As shown in Figure~\ref{fig:attack}, the WLR of $\text{CPA}_{0.1\%}$ is below 1.0005 for \texttt{fft\_a} and \texttt{adaptec1} design. The WER of DW and \sys cells is near 100\%. However, when the placement is not usable like SLA and CPA with larger cell perturbations, the WLR goes much lower. (iii) For the largest placement \texttt{superblue12}, even the smallest perturbation makes the placement unusable like $\text{SLA}_{10}$ and $\text{CPA}_{0.1\%}$. Therefore, the low extraction rate on DW and \sys{} cells is acceptable. (iv) We also highlight that compared to row parity, where some of the cells are not extractable after attacks,  both GW and \sys{} region extraction consistently achieve 100\% WER despite the placement becoming unusable post-attack.


\subsubsection{Constraint Perturbation Attacks (CPA)}
In this attack, cells shift their location along the x- or y-axis if space is available.

\subsubsection{ECO Attacks (ECOA)}
In this attack, the output placement goes through another round of detailed placement from open-source placers like ECO, aiming to remove the watermark. 

\subsubsection{Adaptive Region Attacks (ARA)}
In this attack, the adversary searches for rectangle regions within the placement and perturbs cells within those regions. 


\subsection{Watermark Efficiency}



watermark on top of the optimized placement.
The intelligent property lies in finding constraints; running global placement actually takes less time.
\begin{figure*}[t]
  \begin{center}
       \subfloat[PWLR]{\label{f:pwlr}\includegraphics[width=0.33\linewidth]{figs/pwlr.pdf}}
    \subfloat[RWLR]{\label{f:rwlr}\includegraphics[width=0.33\linewidth]{figs/pwlr.pdf}}
  \subfloat[WER]{\label{f:wer}\includegraphics[width=0.33\linewidth]{figs/wer.pdf}}
\end{center}
  \caption{Performance of the watermarked design under different watermarking frameworks. \textcolor{blue}{Rachel: Can we use a better color scheme here? You can keep blue for row-parity, but use shades of the same color (or related colors) for UniMarks. Using different colors like in the figure makes it seem like different techniques in the first glance.}}
  
  \label{f:results}
  \vspace{-0.4cm}
\end{figure*}

%The watermark region might change with the size of designs, and we add the details of each coefficients in the Parameters column in Table~\ref{tab:ispd2005}-Table~\ref{tab:ispd2019}.

%This entails that the HPWL Ratio should not exceed 1.0005 in comparison to the non-watermarked placement (represented by the black dotted line in Figure~\ref{fig:attack}).
%If this threshold is exceeded, the subsequent manufacturing costs, such as power consumption and efficiency, increases significantly.\
%From left to right along x-axis,
%We consider the swap location attacks where 10 cells and 50 cells are randomly selected to exchange positions with each other; and constraint perturbation attacks where $SLA_{10}$ and $SLA_{50}$ denote 10 cells and 50 cells are randomly selected to exchange positions; $CPA_{0.1\%}$, $CPA_{1\%}$, and $CPA_{10\%}$ mean 0.1\% cells, 1\% cells, and 10\% cells are selected to move along x- or y-axis if there is space. 
 %\rachel{The figure looks much better. Another suggestion to improve it is to use x-axis entires as $SLA_{10}$ instead of SLA (10 cells), and $PCA_{0.1\%}$ instead of PCA (0.1\% cells). If we have space, we can improve readability by making the current 2 x 3 into 3 x 2. Having WLR and WER for one design per row and call it (a) combined. }


\begin{comment}
    \begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/macro_case.pdf}
    \caption{Visualization of Bigblue4, where blue cells are denoted as standard cells and red cells are denoted as macros.}
    \label{fig:macro}
\end{figure}
%, and add the bit sequences along with watermark cells as an additional term to minimize in greedy algorithm in the legalization phase. 
%\rachel {Ratio and percentage don't go together. If you are using ratio - the max value should be 1.0 and not 100\% - Please be consistent and clear on this. If you want to use percentage as 100\%, change to WER - WM Extraction Percentage}
\begin{figure*}[ht]
  \begin{center}
   \subfloat[WLR on \texttt{fft\_a}]{\label{fig:attack_ffta_hpwl}\includegraphics[width=0.32\linewidth]{figs/plot_degradefft_a.pdf}}
   \subfloat[WLR on \texttt{adaptec1}]
   {\label{fig:attack_ada1_hpwl}\includegraphics[width=0.32\linewidth]{figs/plot_degradeadaptec1.pdf}}
    \subfloat[WLR on \texttt{superblue12}]
    {\label{fig:attack_blue4_hpwl}\includegraphics[width=0.32\linewidth]{figs/plot_degradesuperblue12.pdf}}  \\
    \subfloat[WER on \texttt{fft\_a}]
    {\label{fig:attack_ffta_wm}\includegraphics[width=0.32\linewidth]{figs/plot_extractfft_a.pdf}}
   \subfloat[WER on \texttt{adaptec1}]{\label{fig:attack_ada1_wm}\includegraphics[width=0.32\linewidth]{figs/plot_extractadaptec1.pdf}}
    \subfloat[WER on \texttt{superblue12}]{\label{fig:attack_blue4_wm}\includegraphics[width=0.32\linewidth]{figs/plot_extractsuperblue12.pdf}}
  \end{center}
  \vspace{-0.3cm}
  \caption{Considered watermarking schemes' resilience against swap location attack(SLA) and constraint perturbation attack(CPA).}
  \label{fig:attack}

\end{figure*}
\end{comment}
%For a fair comparison with row parity, apart from the \textit{Global Watermarking} that watermarks specific regions, for both \textit{Detailed Watermarking} and \sys{}, we watermark 50 cells and report their HPWL Ratio and WM Extract Ratio. 


\begin{itemize}
    \item  In comparison to DW and row parity, \sys{} demonstrates higher placement and routing quality across all benchmarks. While row parity and DW introduce watermarking during legalization and before detailed placement, significantly reducing performance degradation, \sys{} further enhances the process by identifying regions that contribute less to the overall placement's degradation. As a result, compared with row parity, \sys{} achieves 0.27\%, 1.36\%, and 0.69\% PWLR improvement on ISPD'2005, ISPD'2015, and ISPD'2019 benchmarks; and XX\% and 2.00\% RWLR improvement on ISPD'2015 and ISPD'2019 benchmarks.

   \item   Compared to GW, \sys{} achieves better PWLR and RWLR in most datasets. HPWL across all benchmarks. GW degrades placement performance in ISPD'2005 and ISPD'2019 benchmarks, whereas \sys{} maintains the high-quality results. This is attributed to the second step of \textit{Detailed Watermarking} in \sys{}, which effectively compensates for the overall quality degradation caused by GW.

   \item   For benchmarks where fence regions are included as additional optimization objectives in Table~\ref{tab:ispd2015}, we find the row parity watermarking yields worse PWLR, and some of the designs have WLR degradation of $> 0.5\%$ compared with the original placement, such as \texttt{des\_perf\_b} and \texttt{pci\_bridge32\_a}. \sys{}, however, still maintains high quality with an average WLR of 0.9972. 
    \item  As the number of cells in the design scales up, \sys{} still achieves better placement quality than the baseline row parity~\cite{kahng2001constraint}. For instance, for \texttt{superblue12} in ISPD'2015, \texttt{ispd19test9} and \texttt{ispd19test10} in ISPD'2019 consisting of millions of cells, the WLR of \sys{} is better than that of row parity. We note that there are cases like \texttt{bigblue3} and \texttt{bigblue4} in the ISPD'2005 benchmark where the WLR of \sys{} is higher than row parity. Upon investigation, we found that the reduced quality primarily stems from a large number of macros spreading the placement. Their dense connections cause the degradation to increase. However, as an alternate solution, we found that detailed placement watermarking still has a high extractability and results in only 0.01\% performance degradation, whereas row parity degrades performance by an average of 0.25\% compared with the non-watermarked placements.
\end{itemize}

==> files_backup/6_related.tex <==
%\subsection{VLSI Placement}
%\textcolor{blue}{Rachel: Shouldn't this section be after Introduction or after background? Why is this at the end? It is more appropriate to have a Discussions section at the end.}

%VLSI physical design converts the RTL description in the logic design to the layout representation for manufacturing. The physical design generally consists of five stages. In the first stage, \textbf{floorplanning} defines macros' arrangement and approximate locations in the canvas. Then, \textbf{placement} decides the exact location of the standard cells in the canvas. \textbf{Clock tree synthesis} designs the cell clock distribution network in the cell placement. Next, \textbf{routing} creates paths for electrical signals to connect various components as defined in the netlist. Finally, \textbf{verification} is applied to ensure the functionality of the layout is performed as expected. Among these steps, \textbf{placement} is considered as the fundamental stage in VLSI physical design and has a huge impact on chip performance, power consumption, and area utilization. Many works have proposed to improve the performance of placement or routing algorithms with various techniques. 

%The analytical placement algorithms achieve state-of-the-art by applying force-directed or electrostatics-based formulations~\cite{lin2019dreamplace,lin2020dreamplace,agnesina2020vlsi} to minimize wirelength $W$ with cell density constraints below $\mathcal{D}$. The process of analytical VLSI placement~\cite{qiu2023progress,pawanekar2015nonlinear,agnesina2020vlsi,lin2021routability} consists of three stages: global placement, legalization, and detailed placement. First, global placement generates approximate physical locations for all instances. It primarily mitigates overlaps between instances and induces a rough arrangement by solving an optimization problem. Recent work solves it via gradient-based approaches in DREAMPlace~\cite{lin2019dreamplace} which accelerates ePlace~\cite{lu2015eplace}/RePlAce~\cite{cheng2018replace} via GPU supports.  Second, legalization aligns the instances to predefined rows by conforming to the node specifications.
%It also ensures the power and ground alignments are legal. Finally, detailed placement subtly adjusts the layout and enhances the design quality via meticulous refinement. 
%\textcolor{red}{To Rachel: I don't know if we need to add the machine learning based placement/routing here. Coz reviewer might ask how our wm works on ml-based approaches? But I'm not sure}

%More recent work applies machine learning algorithms like reinforcement learning-based algorithms to place cells properly in the global placement or the floorplanning stage. Azalia Mirhoseini~\textit{et.al.}~\cite{mirhoseini2020chip} proposed to use deep reinforcement learning to place macros on the chip canvas as a sequential decision-making problem. Ruoyu Chen~\textit{et.al.}~\cite{cheng2021joint} further bridges the placement with subsequent routing tasks by including a multi-view embedding model to extract global graph information and local node information.  ChipFormer~\cite{lai2023chipformer} improves the transferability of the reinforcement learning algorithms by exploiting offline placement designs to learn transferable policies more efficiently in a multi-task setting.
%These works perform machine learning algorithms during the global placement stage. Our watermarking frameworks can be used as an add-on co-optimization term during the placement pipeline to enhance the IP protection of these algorithms. 


%\subsection{VSLI Design Watermarking}
%Watermarking primarily serves as an essential method to protect intelligent property in the long IC supply chain. It provides the origins and authenticates of various components in every stage of the VSLI design. The insertion of the watermark should maintain the functionality of the design while being hard to detect and remove by adversaries. 
%Based on the time the watermarks are inserted, they can be categorized into (i) logic and (ii) physical design watermarking.

\textbf{Logic Watermarking} Designers embed unique signatures into the RTL description of the design or the netlists. The signatures are inserted by adding redundant components to the finite state machine~\cite{5938070,divyanshu2023fsm} or netlists~\cite{yuan2006vlsi}. As the size of the IC components become larger, more recent work proposed to add side-channel information like power consumptions~\cite{becker2010side,das2023psc} or hardware trojans~\cite{8764416} to trigger malicious function as signatures.

\textbf{Physical Design Watermarking} The watermarks are inserted into the layout during the physical design stage. The watermark signatures are usually inserted at the placement or the routing stage to alter the design. A.B. Kahng~\textit{et.al}~\cite{kahng2001constraint} proposed to alter the positions of the standard cells in the placement stage to even or odd rows based on the binary signatures and thus insert watermarks into the design. %It also proposed to limit the way of selected watermark unique signal nets and insert such information as unique signatures. \textcolor{red}{To Rachel: I actually didn't understand how this paper does routing wm. We might need to talk together.} 
%\textcolor{blue}{Rachel: Routing in ASICs is done using metal layers. To go from (x1, y1) to (x2, y2) the path is rectilinear and each of the routed portion is refereed to as 'route segments'. In the row-parity paper, they modify the route segment widths, the spacings between two route lines as well as the topology using parity. Topology is based on the direction of the route segments. You can route 'L' or '7' and they are two different topologies which can be assigned a parity of '0' or '1'.}

%1. Congestive design for routing level wm is very hard, and also adding additional wirelength.
%1. routing wm can also be combined to make layout wm more robust. 

Guangyu Sun~\textit{et.al}~\cite{1613214} proposed to add redundant cells in the placement stage as unique signatures. Nie, T~\textit{et.al}~\cite{1510323} proposed to add redundant wires in the routing stage as unique signatures. However, such redundant cells or wires can be easily removed if adversaries are in the downstream fabricate company and can access the layout. Therefore, a more resilient and robust watermarking scheme for VLSI physical design is needed to protect designer IP better.  


%\subsection{Challenges}

%To effectively defend the threat model without degrading overall layout quality, we identify three challenges:

%\noindent\textbf{Challenge 1: Dense Connections} Due to dense interconnections within the standard cells, randomly changing cell positions or cell connections without considering the overall distribution will result in huge performance degradations. Besides, such dense connections also bring huge computational overhead for constraint-based routing watermarking approaches~\cite{kahng2001constraint,1510323}. 
%Thus, developing an efficient watermarking approach that considers the dense nature of cell connections to minimize negative impacts on the layout quality is crucial.

%\noindent\textbf{Challenge 2: Design Constraints} Current benchmark suites incorporate additional design constraints, such as fence regions, into the design process. However, when adding those design constraints into the design loop, the previous row parity-based approach~\cite{kahng2001constraint} resulted in huge layout quality degradation.
%The resulting watermarking placement exhibited substantial degradation compared to non-watermarked solutions. 
%A more comprehensive approach is required to address these additional design constraints while embedding watermarks effectively.


%\noindent\textbf{Challenges 3: Confidentiality} The watermark within the layout must be confidential to prevent ghost attacks on the watermarked solutions. In the row parity approach~\cite{kahng2001constraint}, adversaries can easily extract another set of watermarked cells and their row identifiers from the layout as ghost watermarks. It is essential to devise a watermarking method that ensures the confidentiality of the watermark, thereby enhancing its security against such attacks.

==> files_backup/7_discussion.tex <==



In this section, we first discuss the performance of \sys{} on watermarking the layouts generated by the timing-driven placement algorithms. As a proof-of-concept, it demonstrated \sys's performance on watermarking physical design algorithms with additional optimization constraints. Then, for the first time, we perform our watermarking algorithm on the commercial designs and report their PPA metrics.  \textcolor{red}{To Rachel: Could you point me to some links for the design? I'm thinking about how to name it to avoid the reviewer saying things like our previous benchmarks are not real-world loll.}
\rachel{Are you referring to open-source designs? You can find lots of designs \href{https://opencores.org/}{here}}



==> files_backup/abstract.tex <==
This paper presents \sys{}, a novel watermarking framework designed to protect the intellectual property (IP) of the integrated circuit (IC) physical design in its long global supply chain.
Design companies invest significant efforts in refining the IC physical design processes to satisfy design specifications and enhance power-performance-area (PPA) metrics. However, the crucial physical design IPs are susceptible to threats such as overbuilding or counterfeiting, resulting in unauthorized use.
\sys{} proposes IP protection by embedding unique watermark signatures during the physical design's placement stage, thereby authenticating IC layout ownership. 
\sys{} watermark insertion has two phases: (i) the \textit{Global Watermarking} identifies the watermarked region and its associated cells with minimal performance deterioration to insert as signatures, and (ii) the \textit{Detailed Watermarking} perturbs cells within the watermarked region to augment the signatures. Ownership is verified by retrieving the signatures from cells in the watermarked region and comparing them with inserted ones. 
Extensive proof-of-concept evaluations validate that \sys{} incurs minimal quality metrics degradation with 100\% watermark extraction rates. 
Furthermore, we systematically categorize potential threats to the watermarked layouts into ghost, denial, and removal attacks, highlighting \sys{}'s robustness to the pertinent attacks. 


%\sys{} targets the insertion of unique watermark signatures into the designer's physical design algorithms that are typically optimized for enhancing the quality of the designed chips. 
%\racheltodo{Including one sentence about potential IP piracy schemes that we try to protect against would help - How others can claim ownership in an illegitimate way.}
%\ruisi{In the physical design process, researchers and engineers spend weeks and months exploring optimized and customized design constraints, which produce less power consumption, better performance, and less area utilization (PPA) in the chip products. \sys{} targets the insertion of unique watermark signatures into the physical design algorithms and provides ownership proof for the generated chip layouts.}
%\rachel{}

==> files_backup/conclusion.tex <==
We present \sys{}, a unified watermarking framework for physical design layout IP protection in supply chains. We first introduce a \textit{Global Watermarking} method that identifies regions with insignificant performance degradation; then, we propose an independent \textit{Detailed Watermarking} technique to insert signatures. Based on these methods, we develop \sys{}, which combines the best attributes of both \textit{Global} and \textit{Detailed Watermarking}, thereby achieving high watermark extraction rates with augmented watermarking strength. Extensive experiments on ISPD'2005~\cite{nam2005ispd2005}, ISPD'2015~\cite{bustany2015ispd}, ISPD'2019~\cite{liu2019ispd}, and ICCAD'2015~\cite{7372671} benchmarks demonstrate that \sys{} successfully inserted watermarked without compromising layout quality. Furthermore, we showcased \sys{}'s resiliency against ghost, denial, and removal attacks through comprehensive security analysis. 
 

==> files_backup/link.tex <==


\hyperlink{https://docs.google.com/presentation/d/1xVcTMXzdqCmRp_I2eJg5BqK78EtaDB7n/edit?usp=sharing&ouid=113017722085653394029&rtpof=true&sd=true}{Fig1}

\hyperlink{https://docs.google.com/presentation/d/1xVcTMXzdqCmRp_I2eJg5BqK78EtaDB7n/edit?usp=sharing&ouid=113017722085653394029&rtpof=true&sd=true}{Fig2}

\hyperlink{https://colab.research.google.com/drive/1dE2ISh1IGwYpOYN_Bg7rfXlTMKRqmVwu?usp=sharing}{Attack Fig}

==> table/all_tab_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h!]
\small
\centering
\resizebox{0.94\textwidth}{!}{%
\begin{tabular}{@{}|ccc|cc|cl|cl|cl|cl|@{}}
\toprule
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & {\color[HTML]{1F1F1F} } & \multicolumn{2}{c|}{{\color[HTML]{1F1F1F} Parameters}} & \multicolumn{2}{c|}{Row Parity~\cite{kahng2001constraint}} & \multicolumn{2}{c|}{GW} & \multicolumn{2}{c|}{DW} & \multicolumn{2}{c|}{\sys} \\ \cmidrule(l){4-13} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Cells}} & \multirow{-2}{*}{{\color[HTML]{1F1F1F} Nets}} & \multicolumn{1}{c|}{Size} & {\color[HTML]{1F1F1F} Stride} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} \\ \midrule
\multicolumn{1}{|c|}{adaptec1} & \multicolumn{1}{c|}{211K} & 221K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{c|}{1.0040} & 100\% & \multicolumn{1}{c|}{1.0004} & 100\% & \multicolumn{1}{c|}{\textbf{0.9999}} & 100\% & \multicolumn{1}{c|}{1.0003} & 100\% \\ \midrule
\multicolumn{1}{|c|}{adaptec2} & \multicolumn{1}{c|}{255K} & 266K & \multicolumn{1}{c|}{60} & 10 & \multicolumn{1}{c|}{1.0007} & 100\% & \multicolumn{1}{c|}{1.0041} & 100\% & \multicolumn{1}{c|}{0.9999} & 100\% & \multicolumn{1}{c|}{\textbf{0.9982}} & 100\% \\ \midrule
\multicolumn{1}{|c|}{adaptec3} & \multicolumn{1}{c|}{452K} & 467K & \multicolumn{1}{c|}{20} & 5 & \multicolumn{1}{c|}{1.0034} & 100\% & \multicolumn{1}{c|}{0.9988} & 100\% & \multicolumn{1}{c|}{1.0004} & 100\% & \multicolumn{1}{c|}{\textbf{0.9859}} & 100\% \\ \midrule
\multicolumn{1}{|c|}{adaptec4} & \multicolumn{1}{c|}{496K} & 516K & \multicolumn{1}{c|}{30} & 10 & \multicolumn{1}{c|}{1.0019} & 100\% & \multicolumn{1}{c|}{0.9992} & 100\% & \multicolumn{1}{c|}{1.0000} & 100\% & \multicolumn{1}{c|}{\textbf{0.9993}} & 100\% \\ \midrule
\multicolumn{1}{|c|}{bigblue1} & \multicolumn{1}{c|}{278K} & 284K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{c|}{1.0013} & 100\% & \multicolumn{1}{c|}{0.9972} & 100\% & \multicolumn{1}{c|}{1.0000} & 100\% & \multicolumn{1}{c|}{\textbf{0.9971}} & 100\% \\ \midrule
\multicolumn{1}{|c|}{bigblue2} & \multicolumn{1}{c|}{558K} & 577K & \multicolumn{1}{c|}{200} & 10 & \multicolumn{1}{c|}{1.0034} & 100\% & \multicolumn{1}{c|}{1.0033} & 100\% & \multicolumn{1}{c|}{1.0047} & 100\% & \multicolumn{1}{c|}{\textbf{1.0033}} & 100\% \\ \midrule
\multicolumn{1}{|c|}{bigblue3} & \multicolumn{1}{c|}{1097K} & 1123K & \multicolumn{1}{c|}{200} & 10 & \multicolumn{1}{c|}{1.0031} & 100\% & \multicolumn{1}{c|}{1.0099} & 100\% & \multicolumn{1}{c|}{\textbf{1.0001}} & 100\% & \multicolumn{1}{c|}{1.0099} & 100\% \\ \midrule
\multicolumn{1}{|c|}{bigblue4} & \multicolumn{1}{c|}{2177K} & 2230K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{c|}{1.0019} & 100\% & \multicolumn{1}{c|}{1.0034} & 100\% & \multicolumn{1}{c|}{\textbf{1.0001}} & 100\% & \multicolumn{1}{c|}{1.0034} & 100\% \\ \midrule
\multicolumn{3}{|c|}{Average: All Designs} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{1.0024} & 100\% & \multicolumn{1}{c|}{1.0020} & 100\% & \multicolumn{1}{c|}{1.0006} & 100\% & \multicolumn{1}{c|}{\textbf{0.9997}} & \textbf{100\%} \\ \bottomrule
\end{tabular}%
} %\vspace{-0.1cm}
\caption{Watermarking performance in ISPD'2005 benchmarks~\cite{nam2005ispd2005}.
}
\label{tab:ispd2005}
\end{table*}

\begin{table*}[h!]
\small
\centering
\resizebox{0.94\textwidth}{!}{%
\begin{tabular}{@{}|lll|cc|ll|ll|ll|ll|@{}}
\toprule
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} }} & \multicolumn{2}{c|}{{\color[HTML]{1F1F1F} Parameters}} & \multicolumn{2}{c|}{Row Parity~\cite{kahng2001constraint}} & \multicolumn{2}{c|}{GW} & \multicolumn{2}{c|}{DW} & \multicolumn{2}{c|}{\sys} \\ \cmidrule(l){4-13} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Cells}} & \multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{1F1F1F} Nets}}} & \multicolumn{1}{c|}{Size} & {\color[HTML]{1F1F1F} Stride} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_des\_perf\_a}} & \multicolumn{1}{l|}{108K} & 115K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0045} & 100\% & \multicolumn{1}{l|}{0.9976} & 100\% & \multicolumn{1}{l|}{0.9994} & 100\% & \multicolumn{1}{l|}{\textbf{0.9972}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_des\_perf\_b}}& \multicolumn{1}{l|}{113K} & 113K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0058} & 100\% & \multicolumn{1}{l|}{0.9930} & 100\% & \multicolumn{1}{l|}{0.9990} & 100\% & \multicolumn{1}{l|}{\textbf{0.9890}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_edit\_dist\_a}} & \multicolumn{1}{l|}{127K} & 134K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0015} & 100\% & \multicolumn{1}{l|}{0.9980} & 100\% & \multicolumn{1}{l|}{0.9998} & 100\% & \multicolumn{1}{l|}{\textbf{0.9980}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_matrix\_mult\_b}} & \multicolumn{1}{l|}{146K} & 152K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0047} & 100\% & \multicolumn{1}{l|}{1.0010} & 100\% & \multicolumn{1}{l|}{1.0002} & 100\% & \multicolumn{1}{l|}{\textbf{0.9994}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_matrix\_mult\_c}} & \multicolumn{1}{l|}{146K} & 152K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0031} & 100\% & \multicolumn{1}{l|}{1.0017} & 100\% & \multicolumn{1}{l|}{0.9990} & 100\% & \multicolumn{1}{l|}{\textbf{0.9963}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_pci\_bridge32\_a} }& \multicolumn{1}{l|}{30K} & 34K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0080} & 100\% & \multicolumn{1}{l|}{1.0361} & 100\% & \multicolumn{1}{l|}{1.0011} & 100\% & \multicolumn{1}{l|}{\textbf{0.9997}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_pci\_bridge32\_b}} & \multicolumn{1}{l|}{29K} & 33K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0069} & 100\% & \multicolumn{1}{l|}{0.9945} & 100\% & \multicolumn{1}{l|}{0.9997} & 100\% & \multicolumn{1}{l|}{\textbf{0.9945}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_superblue11\_a}} & \multicolumn{1}{l|}{926K} & 936K & \multicolumn{1}{c|}{100} & 40 & \multicolumn{1}{l|}{1.0052} & 100\% & \multicolumn{1}{l|}{0.9992} & 100\% & \multicolumn{1}{l|}{0.9995} & 100\% & \multicolumn{1}{l|}{\textbf{0.9986}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{mgc\_superblue16\_a} }& \multicolumn{1}{l|}{680K} & 697K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0030} & 100\% & \multicolumn{1}{l|}{1.0018} & 100\% & \multicolumn{1}{l|}{\textbf{1.0000}} & 100\% & \multicolumn{1}{l|}{1.0017} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_des\_perf\_1} & \multicolumn{1}{l|}{113K} & 113K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0035} & 100\% & \multicolumn{1}{l|}{1.0031} & 100\% & \multicolumn{1}{l|}{1.0042} & 100\% & \multicolumn{1}{l|}{\textbf{0.9964}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_fft\_1} & \multicolumn{1}{l|}{35K} & 33K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0017} & 100\% & \multicolumn{1}{l|}{0.9671} & 100\% & \multicolumn{1}{l|}{1.0026} & 100\% & \multicolumn{1}{l|}{\textbf{0.9671}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_fft\_2} & \multicolumn{1}{l|}{35K} & 33K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0050} & 100\% & \multicolumn{1}{l|}{0.9767} & 100\% & \multicolumn{1}{l|}{1.0027} & 100\% & \multicolumn{1}{l|}{\textbf{0.9767}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_fft\_a} & \multicolumn{1}{l|}{34K} & 32K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0121} & 100\% & \multicolumn{1}{l|}{0.9939} & 100\% & \multicolumn{1}{l|}{1.0075} & 100\% & \multicolumn{1}{l|}{\textbf{0.9939}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_fft\_b} & \multicolumn{1}{l|}{34K} & 32K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0018} & 100\% & \multicolumn{1}{l|}{0.9924} & 100\% & \multicolumn{1}{l|}{0.9991} & 100\% & \multicolumn{1}{l|}{\textbf{0.9924}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_matrix\_mult\_1} & \multicolumn{1}{l|}{160K} & 159K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0050} & 100\% & \multicolumn{1}{l|}{0.9753} & 100\% & \multicolumn{1}{l|}{1.0004} & 100\% & \multicolumn{1}{l|}{\textbf{0.9753}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_matrix\_mult\_2} & \multicolumn{1}{l|}{160K} & 159K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0033} & 100\% & \multicolumn{1}{l|}{0.9867} & 100\% & \multicolumn{1}{l|}{0.9990} & 100\% & \multicolumn{1}{l|}{\textbf{0.9852}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_matrix\_mult\_a} & \multicolumn{1}{l|}{154K} & 154K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0037} & 100\% & \multicolumn{1}{l|}{0.9973} & 100\% & \multicolumn{1}{l|}{1.0005} & 100\% & \multicolumn{1}{l|}{\textbf{0.9973}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_superblue12} & \multicolumn{1}{l|}{1293K} & 1293K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0031} & 100\% & \multicolumn{1}{l|}{1.0036} & 100\% & \multicolumn{1}{l|}{0.9994} & 100\% & \multicolumn{1}{l|}{\textbf{0.9854}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_superblue14} & \multicolumn{1}{l|}{634k} & 620k & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0020} & 100\% & \multicolumn{1}{l|}{\textbf{0.9851}} & 100\% & \multicolumn{1}{l|}{1.0001} & 100\% & \multicolumn{1}{l|}{0.9887} & 100\% \\ \midrule
\multicolumn{1}{|l|}{mgc\_superblue19} & \multicolumn{1}{l|}{522K} & 512K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0025} & 100\% & \multicolumn{1}{l|}{0.9881} & 100\% & \multicolumn{1}{l|}{1.0003} & 100\% & \multicolumn{1}{l|}{\textbf{0.9814}} & 100\% \\ \midrule
\multicolumn{3}{|c|}{Average: Fence Region Designs} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{l|}{1.0048} & 100\% & \multicolumn{1}{l|}{1.0025} & 100\% & \multicolumn{1}{l|}{0.9997} & 100\% & \multicolumn{1}{l|}{\textbf{0.9972}} & \textbf{100\%} \\ \midrule
\multicolumn{3}{|c|}{Average: All Designs} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{l|}{1.0043} & 100\% & \multicolumn{1}{l|}{0.9946} & 100\% & \multicolumn{1}{l|}{1.0007} & 100\% & \multicolumn{1}{l|}{\textbf{0.9907}} & \textbf{100\%} \\ \bottomrule
\end{tabular}%
} 
%\vspace{-0.1cm}
\caption{Watermarking performance in ISPD'2015 benchmarks~\cite{bustany2015ispd}. The designs in blue have fence regions in the placement.}
\label{tab:ispd2015}

\end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h!]
\small
\centering
\resizebox{0.94\textwidth}{!}{%
\begin{tabular}{@{}|lll|cc|ll|ll|ll|ll|@{}}
\toprule
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} }} & \multicolumn{2}{c|}{{\color[HTML]{1F1F1F} Parameters}} & \multicolumn{2}{c|}{Row Parity~\cite{kahng2001constraint}} & \multicolumn{2}{c|}{GW} & \multicolumn{2}{c|}{DW} & \multicolumn{2}{c|}{\sys} \\ \cmidrule(l){4-13} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Cells}} & \multicolumn{1}{c|}{\multirow{-2}{*}{{\color[HTML]{1F1F1F} Nets}}} & \multicolumn{1}{c|}{Size} & {\color[HTML]{1F1F1F} Stride} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} & \multicolumn{1}{c|}{WLR $\downarrow$} & \multicolumn{1}{c|}{WER $\uparrow$} \\ \midrule
\multicolumn{1}{|l|}{ispd19test1} & \multicolumn{1}{l|}{9K} & 3K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0060} & 100\% & \multicolumn{1}{l|}{0.9995} & 100\% & \multicolumn{1}{l|}{1.0023} & 100\% & \multicolumn{1}{l|}{\textbf{0.9955}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test2} & \multicolumn{1}{l|}{73K} & 72K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0184} & 100\% & \multicolumn{1}{l|}{1.0007} & 100\% & \multicolumn{1}{l|}{1.0021} & 100\% & \multicolumn{1}{l|}{\textbf{0.9988}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test3} & \multicolumn{1}{l|}{8K} & 9K & \multicolumn{1}{c|}{10} & 1 & \multicolumn{1}{l|}{1.0000} & 100\% & \multicolumn{1}{l|}{0.9997} & 100\% & \multicolumn{1}{l|}{0.9961} & 100\% & \multicolumn{1}{l|}{\textbf{0.9902}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test4} & \multicolumn{1}{l|}{151K} & 146K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0017} & 100\% & \multicolumn{1}{l|}{0.9957} & 100\% & \multicolumn{1}{l|}{0.9998} & 100\% & \multicolumn{1}{l|}{\textbf{0.9957}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{\textcolor{blue}{ispd19test5} }& \multicolumn{1}{l|}{29K} & 29K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0102} & 100\% & \multicolumn{1}{l|}{\textbf{0.9990}} & 100\% & \multicolumn{1}{l|}{0.9996} & 100\% & \multicolumn{1}{l|}{1.0013} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test6} & \multicolumn{1}{l|}{181K} & 180K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0032} & 100\% & \multicolumn{1}{l|}{1.0040} & 100\% & \multicolumn{1}{l|}{\textbf{1.0001}} & 100\% & \multicolumn{1}{l|}{1.0023} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test7} & \multicolumn{1}{l|}{362K} & 359K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0028} & 100\% & \multicolumn{1}{l|}{1.0181} & 100\% & \multicolumn{1}{l|}{\textbf{1.0000}} & 100\% & \multicolumn{1}{l|}{1.0182} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test8} & \multicolumn{1}{l|}{543K} & 538K & \multicolumn{1}{c|}{50} & 10 & \multicolumn{1}{l|}{1.0001} & 100\% & \multicolumn{1}{l|}{0.9961} & 100\% & \multicolumn{1}{l|}{0.9999} & 100\% & \multicolumn{1}{l|}{\textbf{0.9961}} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test9} & \multicolumn{1}{l|}{903K} & 895K & \multicolumn{1}{c|}{200} & 20 & \multicolumn{1}{l|}{1.0072} & 100\% & \multicolumn{1}{l|}{1.0023} & 100\% & \multicolumn{1}{l|}{\textbf{1.0009}} & 100\% & \multicolumn{1}{l|}{1.0023} & 100\% \\ \midrule
\multicolumn{1}{|l|}{ispd19test10} & \multicolumn{1}{l|}{903K} & 895K & \multicolumn{1}{c|}{10} & 5 & \multicolumn{1}{l|}{1.0025} & 100\% & \multicolumn{1}{l|}{0.9972} & 100\% & \multicolumn{1}{l|}{0.9999} & 100\% & \multicolumn{1}{l|}{\textbf{0.9972}} & 100\% \\ \midrule
\multicolumn{3}{|c|}{Average: All Designs} & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{l|}{1.0052} & 100\% & \multicolumn{1}{l|}{1.0012} & 100\% & \multicolumn{1}{l|}{1.0001} & 100\% & \multicolumn{1}{l|}{\textbf{0.9998}} & \textbf{100\%} \\ \bottomrule
\end{tabular}%
}%\vspace{-0.1cm}
 \caption{Watermarking performance in ISPD'2019 benchmarks~\cite{liu2019ispd}.  The designs in blue have fence regions in the placement.}
\label{tab:ispd2019}
\end{table*}


==> table/all_table3.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}



\begin{table*}[][!htbp]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{Row Parity} & \multicolumn{2}{c|}{\sys: GW} & \multicolumn{2}{c|}{\sys: DW} & \multicolumn{2}{c|}{\sys} \\ \cline{2-9} 
\multirow{-2}{*}{Design} & \multicolumn{1}{c|}{PWLR   $\downarrow$} & RWLR $\downarrow$ & \multicolumn{1}{c|}{PWLR $\downarrow$} & RWLR $\downarrow$ & \multicolumn{1}{c|}{PWLR $\downarrow$} & RWLR $\downarrow$ & \multicolumn{1}{c|}{PWLR $\downarrow$} & RWLR $\downarrow$ \\ \hline
{\color[HTML]{4472C4} perf\_a} & \multicolumn{1}{c|}{1.0045} & 1.0155 & \multicolumn{1}{c|}{0.9976} & 0.9873 & \multicolumn{1}{c|}{0.9994} & 1.0003 & \multicolumn{1}{c|}{\textbf{0.9972}} & \textbf{0.9873} \\ \hline
{\color[HTML]{4472C4} perf\_b} & \multicolumn{1}{c|}{1.0058} & 1.0267 & \multicolumn{1}{c|}{0.9930} & 0.9901 & \multicolumn{1}{c|}{0.9990} & 1.0002 & \multicolumn{1}{c|}{\textbf{0.9890}} & \textbf{0.9901} \\ \hline
{\color[HTML]{4472C4} dist\_a} & \multicolumn{1}{c|}{1.0015} & 0.9999 & \multicolumn{1}{c|}{1.0004} & 1.0052 & \multicolumn{1}{c|}{0.9998} & 1.0005 & \multicolumn{1}{c|}{\textbf{1.0004}} & \textbf{1.0052} \\ \hline
{\color[HTML]{4472C4} mult\_b} & \multicolumn{1}{c|}{1.0047} & 1.0199 & \multicolumn{1}{c|}{1.0010} & 1.0028 & \multicolumn{1}{c|}{1.0002} & 1.0044 & \multicolumn{1}{c|}{\textbf{0.9994}} & \textbf{1.0028} \\ \hline
{\color[HTML]{4472C4} mult\_c} & \multicolumn{1}{c|}{1.0031} & 1.0252 & \multicolumn{1}{c|}{1.0017} & 0.9979 & \multicolumn{1}{c|}{0.9990} & 1.0020 & \multicolumn{1}{c|}{\textbf{0.9963}} & \textbf{0.9979} \\ \hline
{\color[HTML]{4472C4} pci\_a} & \multicolumn{1}{c|}{1.0080} & 1.0340 & \multicolumn{1}{c|}{1.0361} & 1.0048 & \multicolumn{1}{c|}{1.0011} & 1.0021 & \multicolumn{1}{c|}{\textbf{0.9997}} & \textbf{0.9950} \\ \hline
{\color[HTML]{4472C4} pci\_b} & \multicolumn{1}{c|}{1.0069} & 1.1173 & \multicolumn{1}{c|}{0.9951} & 1.0026 & \multicolumn{1}{c|}{0.9997} & 1.0008 & \multicolumn{1}{c|}{\textbf{0.9951}} & \textbf{1.0026} \\ \hline
{\color[HTML]{4472C4} superblue11} & \multicolumn{1}{c|}{1.0052} & 1.0344 & \multicolumn{1}{c|}{0.9992} & 0.9992 & \multicolumn{1}{c|}{0.9995} & 1.0005 & \multicolumn{1}{c|}{\textbf{0.9986}} & \textbf{0.9992} \\ \hline
{\color[HTML]{4472C4} superblue16} & \multicolumn{1}{c|}{1.0030} & 1.0210 & \multicolumn{1}{c|}{1.0018} & 1.0204 & \multicolumn{1}{c|}{\textbf{1.0000}} & \textbf{1.0000} & \multicolumn{1}{c|}{1.0017} & 1.0204 \\ \hline
perf\_1 & \multicolumn{1}{c|}{1.0035} & 1.0199 & \multicolumn{1}{c|}{1.0031} & 0.9973 & \multicolumn{1}{c|}{1.0042} & 1.0019 & \multicolumn{1}{c|}{\textbf{0.9964}} & \textbf{0.9973} \\ \hline
fft\_1 & \multicolumn{1}{c|}{1.0017} & 1.0260 & \multicolumn{1}{c|}{0.9671} & 0.9673 & \multicolumn{1}{c|}{1.0026} & 0.9975 & \multicolumn{1}{c|}{\textbf{0.9671}} & \textbf{0.9673} \\ \hline
fft\_2 & \multicolumn{1}{c|}{1.0050} & 1.0260 & \multicolumn{1}{c|}{0.9767} & 0.9770 & \multicolumn{1}{c|}{1.0027} & 0.9996 & \multicolumn{1}{c|}{\textbf{0.9767}} & \textbf{0.9770} \\ \hline
fft\_a & \multicolumn{1}{c|}{1.0121} & 1.0200 & \multicolumn{1}{c|}{0.9939} & 0.9895 & \multicolumn{1}{c|}{1.0075} & 1.0094 & \multicolumn{1}{c|}{\textbf{0.9939}} & \textbf{0.9895} \\ \hline
fft\_b & \multicolumn{1}{c|}{1.0018} & 1.0075 & \multicolumn{1}{c|}{0.9909} & 0.9890 & \multicolumn{1}{c|}{0.9991} & 1.0036 & \multicolumn{1}{c|}{\textbf{0.9909}} & \textbf{0.9890} \\ \hline
mult\_1 & \multicolumn{1}{c|}{1.0050} & 1.0238 & \multicolumn{1}{c|}{0.9753} & 0.9744 & \multicolumn{1}{c|}{1.0004} & 1.0008 & \multicolumn{1}{c|}{\textbf{0.9753}} & \textbf{0.9744} \\ \hline
mult\_2 & \multicolumn{1}{c|}{1.0033} & 1.0199 & \multicolumn{1}{c|}{0.9867} & 0.9900 & \multicolumn{1}{c|}{0.9990} & 0.9992 & \multicolumn{1}{c|}{\textbf{0.9852}} & \textbf{0.9900} \\ \hline
mult\_a & \multicolumn{1}{c|}{1.0037} & 1.0105 & \multicolumn{1}{c|}{0.9973} & 0.9916 & \multicolumn{1}{c|}{1.0005} & 0.9958 & \multicolumn{1}{c|}{\textbf{0.9973}} & \textbf{0.9916} \\ \hline
superblue12 & \multicolumn{1}{c|}{1.0031} & 1.0067 & \multicolumn{1}{c|}{1.0036} & 0.9732 & \multicolumn{1}{c|}{0.9994} & 0.9942 & \multicolumn{1}{c|}{\textbf{0.9854}} & \textbf{0.9732} \\ \hline
superblue14 & \multicolumn{1}{c|}{1.0020} & 1.0057 & \multicolumn{1}{c|}{\textbf{0.9851}} & 0.9867 & \multicolumn{1}{c|}{1.0001} & 1.0000 & \multicolumn{1}{c|}{0.9887} & \textbf{0.9867} \\ \hline
superblue19 & \multicolumn{1}{c|}{1.0025} & 1.0077 & \multicolumn{1}{c|}{0.9881} & 0.9809 & \multicolumn{1}{c|}{1.0003} & 1.0001 & \multicolumn{1}{c|}{\textbf{0.9814}} & \textbf{0.9809} \\ \hline
{\color[HTML]{4472C4} Average: FR} & \multicolumn{1}{c|}{1.0047} & 1.0322 & \multicolumn{1}{c|}{1.00280823} & 1.0011 & \multicolumn{1}{c|}{0.9997} & 1.0012 & \multicolumn{1}{c|}{\textbf{0.9975}} & \textbf{1.0000} \\ \hline
Average: All & \multicolumn{1}{c|}{1.0043} & 1.0231 & \multicolumn{1}{c|}{0.9946} & 0.9913 & \multicolumn{1}{c|}{1.0007} & 1.0006 & \multicolumn{1}{c|}{\textbf{0.9908}} & \textbf{0.9908} \\ \hline
\end{tabular}%
}
\caption{Performance in ISPD'2015 benchmarks~\cite{bustany2015ispd}. All the design watermarks are successfully extracted, i.e., WER = 100\% for all designs.The PWLR and RWLR are the improvement rates over non-watermarked designs. FR is short for fence region.}
\label{tab:ispd2015}
\end{table*}


==> table/attack_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}|c|c|cc|cc|cc|cc|cc|@{}}
\toprule
\multirow{2}{*}{Design} & \multirow{2}{*}{WM} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SLA (10 Cells)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SLA (50 Cells)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}PA (0.1\%)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}PA (1\%)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}PA (10\%)\end{tabular}} \\ \cmidrule(l){3-12} 
 &  & \multicolumn{1}{c|}{WL} & WER & \multicolumn{1}{c|}{WLL} & WER & \multicolumn{1}{c|}{WL} & WER & \multicolumn{1}{c|}{WL} & WER & \multicolumn{1}{c|}{WL} & WER \\ \midrule
\multirow{5}{*}{fft\_a} & \sys{} Region & \multicolumn{1}{c|}{\multirow{2}{*}{1.0021}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0021}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{0.9939}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{0.9946}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0021}} & 100\% \\ \cmidrule(lr){2-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(lr){10-10} \cmidrule(l){12-12} 
 & \sys{} Dist & \multicolumn{1}{c|}{} & 66\% & \multicolumn{1}{c|}{} & 66\% & \multicolumn{1}{c|}{} & 100\% & \multicolumn{1}{c|}{} & 100\% & \multicolumn{1}{c|}{} & 66\% \\ \cmidrule(l){2-12} 
 & GW & \multicolumn{1}{c|}{1.0021} & 100\% & \multicolumn{1}{c|}{1.0021} & 100\% & \multicolumn{1}{c|}{0.9939} & 100\% & \multicolumn{1}{c|}{0.9947} & 100\% & \multicolumn{1}{c|}{1.0021} & 100\% \\ \cmidrule(l){2-12} 
 & DW & \multicolumn{1}{c|}{1.0381} & 66\% & \multicolumn{1}{c|}{1.1763} & 66\% & \multicolumn{1}{c|}{1.0081} & 100\% & \multicolumn{1}{c|}{1.0192} & 62\% & \multicolumn{1}{c|}{1.0249} & 57.99\% \\ \cmidrule(l){2-12} 
 & RP & \multicolumn{1}{c|}{1.0375} & 88\% & \multicolumn{1}{c|}{1.1761} & 88\% & \multicolumn{1}{c|}{1.0142} & 100\% & \multicolumn{1}{c|}{1.0189} & 92\% & \multicolumn{1}{c|}{1.0256} & 90\% \\ \midrule
\multirow{5}{*}{adaptec1} & \sys{} Region & \multicolumn{1}{c|}{\multirow{2}{*}{1.0161}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0161}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0003}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0161}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0161}} & 100\% \\ \cmidrule(lr){2-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(lr){10-10} \cmidrule(l){12-12} 
 & \sys{} Dist & \multicolumn{1}{c|}{} & 10\% & \multicolumn{1}{c|}{} & 10\% & \multicolumn{1}{c|}{} & 98\% & \multicolumn{1}{c|}{} & 10\% & \multicolumn{1}{c|}{} & 10\% \\ \cmidrule(l){2-12} 
 & GW & \multicolumn{1}{c|}{1.0161} & 100\% & \multicolumn{1}{c|}{1.0161} & 100\% & \multicolumn{1}{c|}{1.0003} & 100\% & \multicolumn{1}{c|}{1.0161} & 100\% & \multicolumn{1}{c|}{1.0161} & 100\% \\ \cmidrule(l){2-12} 
 & DW & \multicolumn{1}{c|}{1.0161} & 48\% & \multicolumn{1}{c|}{1.0261} & 50\% & \multicolumn{1}{c|}{0.9998} & 100\% & \multicolumn{1}{c|}{1.0132} & 42\% & \multicolumn{1}{c|}{1.0129} & 22\% \\ \cmidrule(l){2-12} 
 & RP & \multicolumn{1}{c|}{1.0293} & 96\% & \multicolumn{1}{c|}{1.0403} & 96\% & \multicolumn{1}{c|}{1.0165} & 100\% & \multicolumn{1}{c|}{1.0263} & 98\% & \multicolumn{1}{c|}{1.0276} & 96\% \\ \midrule
\multirow{5}{*}{bigblue 4} & \sys{} Region & \multicolumn{1}{c|}{\multirow{2}{*}{1.0179}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0179}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0179}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0179}} & 100\% & \multicolumn{1}{c|}{\multirow{2}{*}{1.0179}} & 100\% \\ \cmidrule(lr){2-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(lr){10-10} \cmidrule(l){12-12} 
 & \sys{} Dist & \multicolumn{1}{c|}{} & 28\% & \multicolumn{1}{c|}{} & 28\% & \multicolumn{1}{c|}{} & 28\% & \multicolumn{1}{c|}{} & 28\% & \multicolumn{1}{c|}{} & 28\% \\ \cmidrule(l){2-12} 
 & GW & \multicolumn{1}{c|}{1.0179} & 100\% & \multicolumn{1}{c|}{1.0179} & 100\% & \multicolumn{1}{c|}{1.0179} & 100\% & \multicolumn{1}{c|}{1.0179} & 100\% & \multicolumn{1}{c|}{1.0179} & 100\% \\ \cmidrule(l){2-12} 
 & DW & \multicolumn{1}{c|}{1.0051} & 64\% & \multicolumn{1}{c|}{1.0092} & 66\% & \multicolumn{1}{c|}{1.0041} & 68\% & \multicolumn{1}{c|}{1.0043} & 68\% & \multicolumn{1}{c|}{1.0050} & 40\% \\ \cmidrule(l){2-12} 
 & RP & \multicolumn{1}{c|}{1.0102} & 100\% & \multicolumn{1}{c|}{1.0142} & 100\% & \multicolumn{1}{c|}{1.0092} & 98\% & \multicolumn{1}{c|}{1.0095} & 96\% & \multicolumn{1}{c|}{1.0108} & 94\% \\ \bottomrule
\end{tabular}%
}
\caption{Watermark scheme under different attack}
\label{tab:attack}
\end{table*}

==> table/iccad2015_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Design} & \multicolumn{3}{c|}{Row Parity} & \multicolumn{3}{c|}{\sys: GW} & \multicolumn{3}{c|}{\sys: DW} & \multicolumn{3}{c|}{\sys} \\ \cline{2-13} 
 & \multicolumn{1}{c|}{TNSR $\downarrow$} & \multicolumn{1}{c|}{WNSR $\downarrow$} & PWLR $\downarrow$ & \multicolumn{1}{c|}{TNSR $\downarrow$} & \multicolumn{1}{c|}{WNSR $\downarrow$} & PWLR $\downarrow$ & \multicolumn{1}{c|}{TNSR $\downarrow$} & \multicolumn{1}{c|}{WNSR $\downarrow$} & PWLR $\downarrow$ & \multicolumn{1}{c|}{TNSR $\downarrow$} & \multicolumn{1}{c|}{WNSR $\downarrow$} & PWLR $\downarrow$ \\ \hline
 \hline 
superblue1 & \multicolumn{1}{c|}{1.0053} & \multicolumn{1}{c|}{1.0094} & \textbf{1.0095} & \multicolumn{1}{c|}{0.9001} & \multicolumn{1}{c|}{\textbf{0.8514}} & 1.0026 & \multicolumn{1}{c|}{1.0256} & \multicolumn{1}{c|}{1.0249} & 1.0102 & \multicolumn{1}{c|}{\textbf{0.8283}} & \multicolumn{1}{c|}{1.2939} & 1.0032 \\ \hline
superblue3 & \multicolumn{1}{c|}{1.0053} & \multicolumn{1}{c|}{1.0176} & 1.0043 & \multicolumn{1}{c|}{\textbf{0.9302}} & \multicolumn{1}{c|}{\textbf{0.9029}} & 0.9999 & \multicolumn{1}{c|}{1.0035} & \multicolumn{1}{c|}{0.9884} & 1.0044 & \multicolumn{1}{c|}{0.9363} & \multicolumn{1}{c|}{0.9047} & \textbf{0.9999} \\ \hline
superblue4 & \multicolumn{1}{c|}{1.1299} & \multicolumn{1}{c|}{0.9914} & 1.0122 & \multicolumn{1}{c|}{\textbf{0.9037}} & \multicolumn{1}{c|}{\textbf{0.9370}} & 1.0019 & \multicolumn{1}{c|}{0.9554} & \multicolumn{1}{c|}{0.9930} & 1.0118 & \multicolumn{1}{c|}{0.9221} & \multicolumn{1}{c|}{1.0094} & \textbf{1.0015} \\ \hline
superblue5 & \multicolumn{1}{c|}{0.9801} & \multicolumn{1}{c|}{\textbf{0.9887}} & 1.0039 & \multicolumn{1}{c|}{0.9159} & \multicolumn{1}{c|}{1.0001} & \textbf{1.0008} & \multicolumn{1}{c|}{0.9922} & \multicolumn{1}{c|}{0.9959} & 1.0050 & \multicolumn{1}{c|}{\textbf{0.9159}} & \multicolumn{1}{c|}{1.0508} & 1.0087 \\ \hline
superblue7 & \multicolumn{1}{c|}{0.9801} & \multicolumn{1}{c|}{0.9932} & 1.0079 & \multicolumn{1}{c|}{\textbf{0.9584}} & \multicolumn{1}{c|}{0.9758} & \textbf{0.9946} & \multicolumn{1}{c|}{0.9934} & \multicolumn{1}{c|}{1.0199} & 1.0081 & \multicolumn{1}{c|}{0.9636} & \multicolumn{1}{c|}{\textbf{0.9727}} & 1.0026 \\ \hline
superblue10 & \multicolumn{1}{c|}{1.0099} & \multicolumn{1}{c|}{\textbf{1.0041}} & 1.0072 & \multicolumn{1}{c|}{1.0069} & \multicolumn{1}{c|}{1.0072} & \textbf{1.0049} & \multicolumn{1}{c|}{\textbf{1.0058}} & \multicolumn{1}{c|}{1.0068} & 1.0055 & \multicolumn{1}{c|}{1.0069} & \multicolumn{1}{c|}{1.0072} & 1.0053 \\ \hline
superblue16 & \multicolumn{1}{c|}{0.9814} & \multicolumn{1}{c|}{1.1271} & 1.0061 & \multicolumn{1}{c|}{1.0166} & \multicolumn{1}{c|}{1.0473} & 0.9976 & \multicolumn{1}{c|}{\textbf{0.9060}} & \multicolumn{1}{c|}{1.3485} & \textbf{1.0004} & \multicolumn{1}{c|}{1.0069} & \multicolumn{1}{c|}{\textbf{1.0072}} & 1.0044 \\ \hline
superblue18 & \multicolumn{1}{c|}{1.0068} & \multicolumn{1}{c|}{0.9965} & 1.0059 & \multicolumn{1}{c|}{0.9337} & \multicolumn{1}{c|}{\textbf{0.9403}} & 1.0058 & \multicolumn{1}{c|}{1.0014} & \multicolumn{1}{c|}{1.0002} & 1.0059 & \multicolumn{1}{c|}{\textbf{0.9254}} & \multicolumn{1}{c|}{0.9449} & \textbf{1.0035} \\ \hline
\hline
Average & \multicolumn{1}{c|}{1.0114} & \multicolumn{1}{c|}{1.0151} & 1.0071 & \multicolumn{1}{c|}{0.9448} & \multicolumn{1}{c|}{\textbf{0.9559}} & \textbf{1.0022} & \multicolumn{1}{c|}{0.9848} & \multicolumn{1}{c|}{1.0418} & 1.0064 & \multicolumn{1}{c|}{\textbf{0.9366}} & \multicolumn{1}{c|}{0.9867} & 1.0036 \\ \hline
\end{tabular}%
}
\caption{ICCAD'2015~\cite{7372671} Timing-driven Placement Watermarking Performance. All the design watermarks are successfully extracted, i.e., WER = 100\% for all designs. The TNSR, WNSR, and WLR are the improvement over non-watermarked designs.}
\label{tab:iccad2015}
\end{table*}
% \rachel{Let's also include placement wirelength ratio here (routing wirelength is optional). If you are comparing to absolute values of WNSR and TNSR, then we should include baseline DREAMPlace4.0 as well.}

==> table/ispd2005.tex <==
\begin{table*}[ht]
\begin{tabular}{@{}|ccc|cc|cc|cc|cc|@{}}
\toprule
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                        & {\color[HTML]{1F1F1F} }                       & \multicolumn{2}{c|}{\sys}                                                                                                                      & \multicolumn{2}{c|}{Global   Watermarking}                                                                                                     & \multicolumn{2}{c|}{Detailed   Watermarking}                                                                                                   & \multicolumn{2}{c|}{Row   Parity}                                                                                                              \\ \cmidrule(l){4-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{cells}} & \multirow{-2}{*}{{\color[HTML]{1F1F1F} nets}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL \\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract \\ Ratio $\uparrow$ \end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL \\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract \\ Ratio $\uparrow$ \end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL \\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract \\ Ratio $\uparrow$ \end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL \\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract \\ Ratio $\uparrow$ \end{tabular} \\ \midrule
\multicolumn{1}{|c|}{adaptec1}                 & \multicolumn{1}{c|}{211K}                    & 221K                                          & \multicolumn{1}{c|}{1.0003}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0004}                                                      & 100\%                                                       & \multicolumn{1}{c|}{\textbf{0.9999}}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0040}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{adaptec2}                 & \multicolumn{1}{c|}{255K}                    & 266K                                          & \multicolumn{1}{c|}{\textbf{0.9982}}                                                     & 100\%                                                       & \multicolumn{1}{c|}{1.0041}                                                      & 100\%                                                       & \multicolumn{1}{c|}{0.9999}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0007}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{adaptec3}                 & \multicolumn{1}{c|}{452K}                    & 467K                                          & \multicolumn{1}{c|}{\textbf{0.9859}}                                                    & 100\%                                                       & \multicolumn{1}{c|}{0.9988}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0004}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0034}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{adaptec4}                 & \multicolumn{1}{c|}{496K}                    & 516K                                          & \multicolumn{1}{c|}{\textbf{0.9993} }                                                     & 100\%                                                       & \multicolumn{1}{c|}{0.9992}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0000}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0019}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{bigblue1}                 & \multicolumn{1}{c|}{278K}                    & 284K                                          & \multicolumn{1}{c|}{\textbf{0.9971}}                                                      & 100\%                                                       & \multicolumn{1}{c|}{0.9972}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0000}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0013}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{bigblue2}                 & \multicolumn{1}{c|}{558K}                    & 577K                                          & \multicolumn{1}{c|}{\textbf{1.0033} }                                                     & 100\%                                                       & \multicolumn{1}{c|}{1.0033}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0047}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0034}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{bigblue3}                 & \multicolumn{1}{c|}{1097K}                   & 1123K                                         & \multicolumn{1}{c|}{1.0099}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0099}                                                      & 100\%                                                       & \multicolumn{1}{c|}{\textbf{1.0001} }                                                     & 100\%                                                       & \multicolumn{1}{c|}{1.0031}                                                      & 100\%                                                       \\ \midrule
\multicolumn{1}{|c|}{bigblue4}                 & \multicolumn{1}{c|}{2177K}                   & 2230K                                         & \multicolumn{1}{c|}{1.0034}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0034}                                                      & 100\%                                                       & \multicolumn{1}{c|}{\textbf{1.0001}}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0019}                                                      & 100\%                                                       \\ \midrule
\multicolumn{3}{|c|}{Average}                                                                                                                 & \multicolumn{1}{c|}{\textbf{0.9997}}                                                      & \textbf{100\%}                                                      & \multicolumn{1}{c|}{1.0020}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0006}                                                      & 100\%                                                       & \multicolumn{1}{c|}{1.0024}                                                      & 100\%                                                       \\ \bottomrule
\end{tabular}
 \caption{Watermarking performance in ISPD 2005 benchmarks}
    \label{tab:ispd2005}
\end{table*}

==> table/ispd2015_1.tex <==
\begin{table*}[ht]
\begin{tabular}{@{}|ccc|cc|cc|cc|cc|@{}}
\toprule
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                        & {\color[HTML]{1F1F1F} }                       & \multicolumn{2}{c|}{\sys}                                                                                                                    & \multicolumn{2}{c|}{Global Watermarking}                                                                                                     & \multicolumn{2}{c|}{Detailed Watermarking}                                                                                                   & \multicolumn{2}{c|}{Row Parity}                                                                                                              \\ \cmidrule(l){4-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{cells}} & \multirow{-2}{*}{{\color[HTML]{1F1F1F} nets}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio$\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio$\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio$\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio$\uparrow$\end{tabular} \\ \midrule
\multicolumn{1}{|c|}{des\_perf\_a}           & \multicolumn{1}{c|}{108K}                    & 115K                                          & \multicolumn{1}{c|}{\textbf{0.9972}  }                                                   & 100\%                                                      & \multicolumn{1}{c|}{0.9976}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9994}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0045}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{des\_perf\_b}           & \multicolumn{1}{c|}{113K}                    & 113K                                          & \multicolumn{1}{c|}{\textbf{0.9890}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9930}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9990}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0058}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{edit\_dist\_a}          & \multicolumn{1}{c|}{127K}                    & 134K                                          & \multicolumn{1}{c|}{\textbf{0.9980}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9980}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9998}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0015}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{matrix\_mult\_b}        & \multicolumn{1}{c|}{146K}                    & 152K                                          & \multicolumn{1}{c|}{\textbf{0.9994}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0010}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0002}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0047}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{matrix\_mult\_c}        & \multicolumn{1}{c|}{146K}                    & 152K                                          & \multicolumn{1}{c|}{\textbf{0.9963}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0017}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9990}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0031}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{pci\_bridge32\_a}       & \multicolumn{1}{c|}{30K}                     & 34K                                           & \multicolumn{1}{c|}{\textbf{0.9997} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{1.0361}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0011}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0080}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{pci\_bridge32\_b}       & \multicolumn{1}{c|}{29K}                     & 33K                                           & \multicolumn{1}{c|}{\textbf{0.9945}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9945}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9997}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0069}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{superblue11\_a}        & \multicolumn{1}{c|}{926K}                    & 936K                                          & \multicolumn{1}{c|}{\textbf{0.9986}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9992}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9995}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0052}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{superblue16\_a}        & \multicolumn{1}{c|}{680K}                    & 697K                                          & \multicolumn{1}{c|}{1.0017}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0018}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{1.0000}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0030}                                                     & 100\%                                                      \\ \hline \midrule
\multicolumn{1}{|c|}{des\_perf\_1}           & \multicolumn{1}{c|}{113K}                    & 113K                                          & \multicolumn{1}{c|}{\textbf{0.9964}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0031}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0042}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0035}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{fft\_1}                & \multicolumn{1}{c|}{35K}                     & 33K                                           & \multicolumn{1}{c|}{\textbf{0.9671} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9671}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0026}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0017}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{fft\_2}                & \multicolumn{1}{c|}{35K}                     & 33K                                           & \multicolumn{1}{c|}{\textbf{0.9767}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9767}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0027}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0050}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{fft\_a}                & \multicolumn{1}{c|}{34K}                     & 32K                                           & \multicolumn{1}{c|}{\textbf{0.9939} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9939}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0075}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0121}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{fft\_b}                & \multicolumn{1}{c|}{34K}                     & 32K                                           & \multicolumn{1}{c|}{\textbf{0.9924}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9924}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9991}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0018}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{matrix\_mult\_1}        & \multicolumn{1}{c|}{160K}                    & 159K                                          & \multicolumn{1}{c|}{\textbf{0.9753}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9753}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0004}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0050}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{matrix\_mult\_2}        & \multicolumn{1}{c|}{160K}                    & 159K                                          & \multicolumn{1}{c|}{\textbf{0.9852} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9867}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9990}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0033}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{matrix\_mult\_a}        & \multicolumn{1}{c|}{154K}                    & 154K                                          & \multicolumn{1}{c|}{\textbf{0.9973}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9973}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0005}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0037}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{superblue12}          & \multicolumn{1}{c|}{1293K}                   & 1293K                                         & \multicolumn{1}{c|}{\textbf{0.9854}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0036}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9994}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0031}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{superblue14}          & \multicolumn{1}{c|}{634k}                    & 620k                                          & \multicolumn{1}{c|}{0.9887}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{0.9851}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0001}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0020}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{superblue19}          & \multicolumn{1}{c|}{522K}                    & 512K                                          & \multicolumn{1}{c|}{\textbf{0.9814} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9881}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0003}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0025}                                                     & 100\%                                                      \\ \midrule
\multicolumn{3}{|c|}{Average}                                                                                                                 & \multicolumn{1}{c|}{\textbf{0.9907}}                                                     & \textbf{100\%}                                                  & \multicolumn{1}{c|}{0.9946}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0007}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0043}                                                     & 100\%                                                      \\ \bottomrule
\end{tabular}
\caption{Watermarking performance in ISPD 2015 benchmarks. The first nine designs in the first half of the table have additional fence region constraints during placement. }
    \label{tab:ispd2015}
\end{table*}

==> table/ispd_2019.tex <==
\begin{table*}[ht]
\begin{tabular}{@{}|ccc|cc|cc|cc|cc|@{}}
\toprule
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                        & {\color[HTML]{1F1F1F} }                       & \multicolumn{2}{c|}{\sys}                                                                                                                    & \multicolumn{2}{c|}{Global Watermarking}                                                                                                     & \multicolumn{2}{c|}{Detailed Watermarking}                                                                                                   & \multicolumn{2}{c|}{Row Parity}                                                                                                              \\ \cmidrule(l){4-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Design}} & \multicolumn{1}{c|}{\multirow{-2}{*}{cells}} & \multirow{-2}{*}{{\color[HTML]{1F1F1F} nets}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio $\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio $\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio $\uparrow$\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}HPWL\\ Degrade $\downarrow$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}WM Extract\\ Ratio $\uparrow$\end{tabular} \\ \midrule
\multicolumn{1}{|c|}{ispd19test1}              & \multicolumn{1}{c|}{9K}                      & 3K                                            & \multicolumn{1}{c|}{\textbf{0.9955} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9995}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0023}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0060}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test2}              & \multicolumn{1}{c|}{73K}                     & 72K                                           & \multicolumn{1}{c|}{\textbf{0.9988} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{1.0007}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0021}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0184}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test3}              & \multicolumn{1}{c|}{8K}                      & 9K                                            & \multicolumn{1}{c|}{\textbf{0.9902} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9997}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9961}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0000}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test4}              & \multicolumn{1}{c|}{151K}                    & 146K                                          & \multicolumn{1}{c|}{\textbf{0.9957}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9957}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9998}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0017}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test5}              & \multicolumn{1}{c|}{29K}                     & 29K                                           & \multicolumn{1}{c|}{1.0013}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{0.9990}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9996}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0102}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test6}              & \multicolumn{1}{c|}{181K}                    & 180K                                          & \multicolumn{1}{c|}{1.0023}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0040}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{1.0001}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0032}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test7}              & \multicolumn{1}{c|}{362K}                    & 359K                                          & \multicolumn{1}{c|}{1.0182}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0181}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{1.0000}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0028}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test8}              & \multicolumn{1}{c|}{543K}                    & 538K                                          & \multicolumn{1}{c|}{\textbf{0.9961} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9961}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9999}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0001}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test9}              & \multicolumn{1}{c|}{903K}                    & 895K                                          & \multicolumn{1}{c|}{1.0023}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0023}                                                     & 100\%                                                      & \multicolumn{1}{c|}{\textbf{1.0009}}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0072}                                                     & 100\%                                                      \\ \midrule
\multicolumn{1}{|c|}{ispd19test10}             & \multicolumn{1}{c|}{903K}                    & 895K                                          & \multicolumn{1}{c|}{\textbf{0.9972} }                                                    & 100\%                                                      & \multicolumn{1}{c|}{0.9972}                                                     & 100\%                                                      & \multicolumn{1}{c|}{0.9999}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0025}                                                     & 100\%                                                      \\ \midrule
\multicolumn{3}{|c|}{Average}                                                                                                                 & \multicolumn{1}{c|}{\textbf{0.9998}}                                                     & \textbf{100\%}                                                 & \multicolumn{1}{c|}{1.0012}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0001}                                                     & 100\%                                                      & \multicolumn{1}{c|}{1.0052}                                                     & 100\%                                                      \\ \bottomrule
\end{tabular}
\caption{Watermarking performance in ISPD 2019 benchmarks}
\label{tab:ispd2019}
\end{table*}
